VersaTune: An Efficient Data Composition Framework for Training Multi-Capability LLMs

As demonstrated by the proprietary Large Language Models (LLMs) such as GPT and Claude series, LLMs have the potential to achieve remarkable proficiency across a wide range of domains, including law, medicine, finance, science, code, etc., all within a single model. These capabilities are further augmented during the Supervised Fine-Tuning (SFT) phase. Despite their potential, existing work mainly focuses on domain-specific enhancements during fine-tuning, the challenge of which lies in catastrophic forgetting of knowledge across other domains. In this study, we introduce **VersaTune**, a novel data composition framework designed for enhancing LLMs' overall multi-domain capabilities during training. We begin with detecting the distribution of domain-specific knowledge within the base model, followed by the training data composition that aligns with the model's existing knowledge distribution. During the subsequent training process, domain weights are dynamically adjusted based on their learnable potential and forgetting degree. Experimental results indicate that VersaTune is effective in multi-domain fostering, with an improvement of 35.21\% in the overall multi-ability performances compared to uniform domain weights. Furthermore, we find that Qwen-2.5-32B + VersaTune even surpasses frontier models, including GPT-4o, Claude3.5-Sonnet and DeepSeek-V3 by 0.86\%, 4.76\% and 4.60\%. Additionally, in scenarios where flexible expansion of a specific domain is required, VersaTune reduces the performance degradation in other domains by 38.77\%, while preserving the training efficacy of the target domain.

==> chapters/deployment.tex <==
\ours is implemented as the data management backend in a scalable manner to facilitate the efficient fine-tuning of our Baichuan-series models~\cite{yang2023baichuan,dong2024baichuanseed}, as demonstrated in \Cref{fig:deployment}. 

\begin{figure}[ht]
    % \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\linewidth]{figures/VersaTune_deployment.pdf}}
    % \includesvg[width=1\linewidth]{figures/VersaTune_deployment.svg}
    % \caption{An illustration of the domain knowledge distribution among models.}
    \caption{Deployment of \ours in Baichuan Inc.}
    \label{fig:deployment}
    \end{center}
    \vskip -0.2in
\end{figure}


% \begin{figure*}[ht]
%     % \vskip 0.2in
%     \begin{center}
%     \centerline{\includegraphics[width=\linewidth]{figures/multi_ability_radar_chart_v3.pdf}}
%     % \includesvg[width=1\linewidth]{figures/multi_ability_radar_chart_v3.svg}
%     \caption{Performances of different models on versatile benchmarks related to various domains under the scenario of effective multi-ability fostering. The background color of the radar chart signifies the domain to which the current benchmark belongs, with reference to the color key provided in \Cref{fig:pipeline}, which includes law, medicine, finance, science, code, and general fields.}
%     \label{fig:domain_expansion_total_appendix}
%     \end{center}
%     \vskip -0.2in
% \end{figure*}


% \begin{figure*}[ht]
%     \vskip -0.2in
%     \begin{center}
%     \centerline{\includegraphics[width=\linewidth]{figures/domain_expansion_ablation.pdf}}
%     \caption{Line chart of the multi-task performances of models across different domains during the domain expansion process. We calculated the average percentage change for both target and non-target domains comparing to the \textit{initial state}. Additionally, we highlighted the performance changes of the \ours at various checkpoints using green numerical annotations.}
%     \label{fig:domain_expansion_ablation}
%     \end{center}
%     \vskip -0.2in
% \end{figure*}



\begin{figure*}[ht]
    % \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\linewidth]{figures/medicine_domain_expansion.pdf}}
    \caption{
    % 以 medicine domain 为例，进行 specific domain expansion 的结果描述图，我们对 fine-tune 过程中每个 epoch 的 checkpoint 进行测试。左边是在 fine-tune 过程中各个 non-target domain 的能力相较于没有微调前的 增长 / 损失 group stacked bar chart，每一组内部，左中右分别是 (1) 100\% specific domain (2) Domain increase with uniform distribution of remainder" 和 (3) VersaTune implemented based on Algorithm。右边的折线图代表了目标的 medicine domain 在 fine-tune 过程中的能力表现相较于没有微调前的增强效果。
    % Domain expansion results, where we take the \textit{medicine} domain as an example.  
    Domain expansion for \textit{medicine} domain of Baichuan series models~\cite{yang2023baichuan,dong2024baichuanseed}. 
    We evaluated checkpoints from each epoch. 
    \textbf{Left (a)} presents the grouped stacked bar chart showing the growth or loss of capabilities in non-target domains compared to the pre-fine-tuning state. Within each group, the left, center, and right bars represent: (1) 100\% specific domain fine-tuning, (2) domain increase with uniform distribution of remainder, and (3) \ours implementation based on \Cref{alg:domain_expansion}. \textbf{Right (b)} features the line chart depicting the enhancement of the medicine domain's capabilities relative to the pre-fine-tuning state.}
    \label{fig:domain_expansion_medicine}
    \end{center}
    \vskip -0.2in
\end{figure*}

\textbf{Performance in Medical Domain.} 
\ours has made significant contributions to the optimization and application of our Baichuan models in the medical domain, enabling the enhancement of capabilities specific to healthcare while maintaining competencies in other domains. 
\Cref{fig:domain_expansion_medicine} illustrates the changes in target domain capabilities and non-target domain capabilities during the fine-tuning process focused on the medical domain. 
% Three interesting phenomena are observed from the outcomes:
\begin{itemize}[leftmargin=*]
    % \item \textbf{Absolute Instance Count vs. Instance Proportion.}
    \item \textbf{Absolute Count vs. Proportion.} 
    Notably, by the \textit{second epoch} of training, the performance degradation across non-target domains tends to be mitigated to some extent, and there is even a positive trend in capability enhancement in some cases. We attribute this phenomenon to the fact that the absolute quantity of instances for each domain, relative to the domain distribution, has a predominant influence on model performance at this stage.
    \item \textbf{Domain Interactions.} 
    Domains are not entirely orthogonal to each other, and there is a degree of mutual reinforcement among them, e.g., enhancing capabilities in the medicine domain can boost performance in the science domain to a certain degree.
    % , as illustrated in \Cref{fig:domain_expansion_medicine}.
    \item \textbf{Domain Mastery Efficiency.} 
    From the slope of the target domain performance increase in \Cref{fig:domain_expansion_medicine} (b), it is evident that the model's efficiency in mastering knowledge of a specific domain diminishes over training. In other words, as training progresses, the model's grasp of the target domain approaches saturation, while its performance on non-target domains declines sharply. Consequently, greater emphasis should be placed on mitigating losses in non-target domains during this phase, aiming to strike a balance between domain expansion and the salvage of capabilities in non-target domains, which is also shown in \Cref{fig:domain_expansion_ablation}.
\end{itemize}

% \begin{table*}[tb]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ccccccccccc}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target Domain\end{tabular}} & \multicolumn{1}{|c|}{Training Step} & \multirow{2}{*}{Method} & \multicolumn{6}{|c|}{Variations in Comprehensive Domains ($\%$)} & \multicolumn{2}{c}{Sum. ($\%$)} \\
% \cline{4-11}
%    & \multicolumn{1}{|c|}{(Epoch)} & & \multicolumn{1}{|c}{Law}  & Medicine  & Finance  & Science  & Code  & \multicolumn{1}{c|}{Other} & \multicolumn{1}{c|}{Target} & Non-Target \\
% \midrule
% \multirow{12}{*}{Law} & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $5.89 & $\color{red} \downarrow $18.82 & $\color{green} \uparrow $14.71 & $\color{red} \downarrow $11.76 & $\color{red} \downarrow $11.18 & $\color{red} \downarrow $5.00 & \multicolumn{1}{|c}{$\color{green} \uparrow $5.89} & \multicolumn{1}{|c}{$\color{red} \downarrow $32.05} \\
%  & \multicolumn{1}{|c|}{1} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $5.38 & $\color{red} \downarrow $7.35 & $\color{green} \uparrow $6.47 & $\color{red} \downarrow $6.58 & $\color{red} \downarrow $0.05 & $\color{green} \uparrow $13.99 & \multicolumn{1}{|c}{$\color{green} \uparrow $5.38} & \multicolumn{1}{|c}{$\color{red} \downarrow $6.48} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $8.25 & $\color{green} \uparrow $6.18 & $\color{green} \uparrow $12.06 & $\color{red} \downarrow $7.65 & $\color{red} \downarrow $6.22 & $\color{green} \uparrow $17.59 & \multicolumn{1}{|c}{$\color{green} \uparrow $8.25} & \multicolumn{1}{|c}{$\color{green} \uparrow $21.96} \\
%   \cline{2-11}
%    & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $35.51 & $\color{red} \downarrow $12.65 & $\color{green} \uparrow $30.59 & $\color{red} \downarrow $4.41 & $\color{red} \downarrow $5.29 & $\color{red} \downarrow $11.76 & \multicolumn{1}{|c}{$\color{green} \uparrow $35.51} & \multicolumn{1}{|c}{$\color{red} \downarrow $3.52} \\
%    & \multicolumn{1}{|c|}{2} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $33.89 & $\color{red} \downarrow $7.94 & $\color{green} \uparrow $26.47 & $\color{red} \downarrow $12.65 & $\color{red} \downarrow $7.65 & $\color{green} \uparrow $5.00 & \multicolumn{1}{|c}{$\color{green} \uparrow $33.89} & \multicolumn{1}{|c}{$\color{green} \uparrow $3.23} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $35.14 & $\color{green} \uparrow $3.53 & $\color{green} \uparrow $18.82 & $\color{red} \downarrow $6.89 & $\color{green} \uparrow $17.06 & $\color{green} \uparrow $13.24 & \multicolumn{1}{|c}{$\color{green} \uparrow $35.14} & \multicolumn{1}{|c}{$\color{green} \uparrow $45.76} \\
%   \cline{2-11}
%    & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $55.84 & $\color{red} \downarrow $17.94 & $\color{green} \uparrow $12.35 & $\color{red} \downarrow $8.82 & $\color{red} \downarrow $23.53 & $\color{red} \downarrow$5.00 & \multicolumn{1}{|c}{$\color{green} \uparrow $55.84} & \multicolumn{1}{|c}{$\color{red} \downarrow $42.94} \\
%     & \multicolumn{1}{|c|}{3} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $52.89 & $\color{red} \downarrow $8.24 & $\color{green} \uparrow $15.00 & $\color{red} \downarrow $12.06 & $\color{red} \downarrow $10.17 & $\color{red} \downarrow $5.12 & \multicolumn{1}{|c}{$\color{green} \uparrow $52.89} & \multicolumn{1}{|c}{$\color{red} \downarrow $20.59} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $51.71 & $\color{red} \downarrow $4.41 & $\color{green} \uparrow $24.71 & $\color{red} \downarrow $5.29 & $\color{green} \uparrow $4.87 & $\color{green} \uparrow $8.42 & \multicolumn{1}{|c}{$\color{green} \uparrow $51.71} & \multicolumn{1}{|c}{$\color{green} \uparrow $29.30} \\
%   \cline{2-11}
%    & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $62.76 & $\color{red} \downarrow $5.00 & $\color{red} \downarrow $2.06 & $\color{red} \downarrow $31.18 & $\color{red} \downarrow $21.76 & $\color{red} \downarrow $12.65 & \multicolumn{1}{|c}{$\color{green} \uparrow $62.76} & \multicolumn{1}{|c}{$\color{red} \downarrow $72.65} \\
%     & \multicolumn{1}{|c|}{4} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $58.12 & $\color{red} \downarrow $9.71 & $\color{green} \uparrow $5.59 & $\color{red} \downarrow $9.41 & $\color{red} \downarrow $10.14 & $\color{red} \downarrow $12.05 & \multicolumn{1}{|c}{$\color{green} \uparrow $58.12} & \multicolumn{1}{|c}{$\color{red} \downarrow $35.72} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & \cellcolor[HTML]{E59191}$\color{green} \uparrow $59.08 & $\color{red} \downarrow $5.59 & $\color{green} \uparrow $13.82 & $\color{red} \downarrow $8.82 & $\color{red} \downarrow $5.61 & $\color{red} \downarrow $6.17 & \multicolumn{1}{|c}{$\color{green} \uparrow $59.08} & \multicolumn{1}{|c}{$\color{red} \downarrow $12.37} \\
% \midrule
% \multirow{12}{*}{Medicine} & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $10.29 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $5.87 & $\color{red} \downarrow $3.82 & $\color{green} \uparrow $24.12 & $\color{red} \downarrow $19.41 & $\color{red} \downarrow $7.35 & \multicolumn{1}{|c}{$\color{green} \uparrow $5.87} & \multicolumn{1}{|c}{$\color{red} \downarrow $16.75} \\
% & \multicolumn{1}{|c|}{1} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $3.82 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $5.36 & $\color{red} \downarrow $5.29 & $\color{green} \uparrow $5.59 & $\color{red} \downarrow $2.65 & $\color{green} \uparrow $6.53 & \multicolumn{1}{|c}{$\color{green} \uparrow $5.36} & \multicolumn{1}{|c}{$\color{green} \uparrow $0.36} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{green} \uparrow $3.53 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $8.17 & $\color{red} \downarrow $7.65 & $\color{green} \uparrow $8.82 & $\color{green} \uparrow $16.47 & $\color{red} \downarrow $6.17 & \multicolumn{1}{|c}{$\color{green} \uparrow $8.17} & \multicolumn{1}{|c}{$\color{green} \uparrow $15.00} \\
% \cline{2-11}
%    & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $18.82 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $40.44 & $\color{red} \downarrow $6.47 & $\color{green} \uparrow $40.00 & $\color{red} \downarrow $7.94 & $\color{red} \downarrow $17.65 & \multicolumn{1}{|c}{$\color{green} \uparrow $40.44} & \multicolumn{1}{|c}{$\color{red} \downarrow $10.88} \\
%    & \multicolumn{1}{|c|}{2} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $7.94 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $33.68 & $\color{red} \downarrow $9.12 & $\color{green} \uparrow $20.59 & $\color{green} \uparrow $4.98 & $\color{red} \downarrow $5.64 & \multicolumn{1}{|c}{$\color{green} \uparrow $33.68} & \multicolumn{1}{|c}{$\color{green} \uparrow $2.87} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{green} \uparrow $12.35 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $35.21 & $\color{green} \uparrow $7.65 & $\color{green} \uparrow $8.84 & $\color{green} \uparrow $16.52 & $\color{green} \uparrow $12.65 & \multicolumn{1}{|c}{$\color{green} \uparrow $35.21} & \multicolumn{1}{|c}{$\color{green} \uparrow $58.01} \\
% \cline{2-11}
% & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $22.35 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $58.78 & $\color{red} \downarrow $8.82 & $\color{green} \uparrow $7.94 & $\color{red} \downarrow $19.12 & $\color{red} \downarrow $10.00 & \multicolumn{1}{|c}{$\color{green} \uparrow $58.78} & \multicolumn{1}{|c}{$\color{red} \downarrow $52.35} \\
%    & \multicolumn{1}{|c|}{3} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $10.46 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $55.69 & $\color{red} \downarrow $14.98 & $\color{green} \uparrow $12.35 & $\color{red} \downarrow $4.41 & $\color{red} \downarrow $14.18 & \multicolumn{1}{|c}{$\color{green} \uparrow $55.69} & \multicolumn{1}{|c}{$\color{red} \downarrow $31.68} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $3.53 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $53.85 & $\color{red} \downarrow $4.52 & $\color{green} \uparrow $17.06 & $\color{green} \uparrow $7.64 & $\color{green} \uparrow $6.03 & \multicolumn{1}{|c}{$\color{green} \uparrow $53.85} & \multicolumn{1}{|c}{$\color{green} \uparrow $22.68} \\
% \cline{2-11}
% & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $27.94 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $64.61 & $\color{red} \downarrow $11.76 & $\color{red} \downarrow $2.35 & $\color{red} \downarrow $21.76 & $\color{red} \downarrow $12.65 & \multicolumn{1}{|c}{$\color{green} \uparrow $64.61} & \multicolumn{1}{|c}{$\color{red} \downarrow $76.46} \\
%    & \multicolumn{1}{|c|}{4} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $13.82 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $58.07 & $\color{red} \downarrow $11.18 & $\color{green} \uparrow $2.35 & $\color{red} \downarrow $6.47 & $\color{red} \downarrow $18.53 & \multicolumn{1}{|c}{$\color{green} \uparrow $58.07} & \multicolumn{1}{|c}{$\color{red} \downarrow $47.65} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $5.59 & \cellcolor[HTML]{FAC5BD}$\color{green} \uparrow $59.81 & $\color{red} \downarrow $4.27 & $\color{green} \uparrow $10.68 & $\color{red} \downarrow $5.94 & $\color{red} \downarrow $10.26 & \multicolumn{1}{|c}{$\color{green} \uparrow $59.81} & \multicolumn{1}{|c}{$\color{red} \downarrow $15.38} \\
% \midrule
% \multirow{12}{*}{Finance} & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{green} \uparrow $20.59 & $\color{red} \downarrow $7.94 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $5.45 & $\color{red} \downarrow $10.29 & $\color{red} \downarrow $12.65 & $\color{red} \downarrow $6.47 & \multicolumn{1}{|c}{$\color{green} \uparrow $5.45} & \multicolumn{1}{|c}{$\color{red} \downarrow $16.76} \\
% & \multicolumn{1}{|c|}{1} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{green} \uparrow $12.05 & $\color{red} \downarrow $7.36 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $8.21 & $\color{red} \downarrow $6.74 & $\color{green} \uparrow $19.41 & $\color{red} \downarrow $8.53 & \multicolumn{1}{|c}{$\color{green} \uparrow $8.21} & \multicolumn{1}{|c}{$\color{green} \uparrow $8.83} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{green} \uparrow $15.07 & $\color{red} \downarrow $4.12 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $10.46 & $\color{green} \uparrow $3.24 & $\color{green} \uparrow $17.06 & $\color{red} \downarrow $8.55 & \multicolumn{1}{|c}{$\color{green} \uparrow $10.46} & \multicolumn{1}{|c}{$\color{green} \uparrow $22.70} \\
% \cline{2-11}
%    & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{green} \uparrow $18.24 & $\color{red} \downarrow $9.71 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $34.97 & $\color{red} \downarrow $9.41 & $\color{green} \uparrow $5.29 & $\color{red} \downarrow $8.82 & \multicolumn{1}{|c}{$\color{green} \uparrow $34.97} & \multicolumn{1}{|c}{$\color{red} \downarrow $4.41} \\
%    & \multicolumn{1}{|c|}{2} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{green} \uparrow $20.59 & $\color{red} \downarrow $7.94 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $31.08 & $\color{red} \downarrow $4.71 & $\color{red} \downarrow $7.69 & $\color{green} \uparrow $4.98 & \multicolumn{1}{|c}{$\color{green} \uparrow $31.08} & \multicolumn{1}{|c}{$\color{green} \uparrow $5.23} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{green} \uparrow $24.70 & $\color{green} \uparrow $7.35 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $33.92 & $\color{red} \downarrow $5.02 & $\color{green} \uparrow $7.08 & $\color{green} \uparrow $10.58 & \multicolumn{1}{|c}{$\color{green} \uparrow $33.92} & \multicolumn{1}{|c}{$\color{green} \uparrow $44.69} \\
% \cline{2-11}
% & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{green} \uparrow $23.53 & $\color{red} \downarrow $9.41 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $55.87 & $\color{red} \downarrow $17.35 & $\color{red} \downarrow $14.71 & $\color{red} \downarrow $7.94 & \multicolumn{1}{|c}{$\color{green} \uparrow $55.87} & \multicolumn{1}{|c}{$\color{red} \downarrow $25.88} \\
%    & \multicolumn{1}{|c|}{3} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{green} \uparrow $15.02 & $\color{red} \downarrow $8.24 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $52.41 & $\color{red} \downarrow $12.06 & $\color{red} \downarrow $10.30 & $\color{red} \downarrow $4.98 & \multicolumn{1}{|c}{$\color{green} \uparrow $52.41} & \multicolumn{1}{|c}{$\color{red} \downarrow $20.56} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{green} \uparrow $24.71 & $\color{red} \downarrow $11.18 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $53.04 & $\color{green} \uparrow $5.29 & $\color{green} \uparrow $4.44 & $\color{green} \uparrow $8.83 & \multicolumn{1}{|c}{$\color{green} \uparrow $53.04} & \multicolumn{1}{|c}{$\color{green} \uparrow $32.09} \\
% \cline{2-11}
%  & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{green} \uparrow $5.00 & $\color{red} \downarrow $9.12 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $62.89 & $\color{red} \downarrow $20.29 & $\color{red} \downarrow $12.94 & $\color{red} \downarrow $21.76 & \multicolumn{1}{|c}{$\color{green} \uparrow $62.89} & \multicolumn{1}{|c}{$\color{red} \downarrow $59.11} \\
%    & \multicolumn{1}{|c|}{4} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{green} \uparrow $5.88 & $\color{red} \downarrow $5.29 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $56.13 & $\color{red} \downarrow $14.09 & $\color{red} \downarrow $13.23 & $\color{red} \downarrow $20.87 & \multicolumn{1}{|c}{$\color{green} \uparrow $56.13} & \multicolumn{1}{|c}{$\color{red} \downarrow $47.60} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{green} \uparrow $14.19 & $\color{red} \downarrow $8.24 & \cellcolor[HTML]{F4DFDA}$\color{green} \uparrow $58.47 & $\color{red} \downarrow $13.24 & $\color{red} \downarrow $8.52 & $\color{red} \downarrow $9.41 & \multicolumn{1}{|c}{$\color{green} \uparrow $58.47} & \multicolumn{1}{|c}{$\color{red} \downarrow $25.22} \\
% \midrule
% \multirow{12}{*}{Science} & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $10.29 & $\color{green} \uparrow $17.06 & $\color{red} \downarrow $3.82 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $6.78 & $\color{red} \downarrow $4.71 & $\color{red} \downarrow $7.35 & \multicolumn{1}{|c}{$\color{green} \uparrow $6.78} & \multicolumn{1}{|c}{$\color{red} \downarrow $9.11} \\
% & \multicolumn{1}{|c|}{1} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $6.76 & $\color{green} \uparrow $17.64 & $\color{red} \downarrow $9.18 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $5.37 & $\color{green} \uparrow $7.05 & $\color{green} \uparrow $4.73 & \multicolumn{1}{|c}{$\color{green} \uparrow $5.37} & \multicolumn{1}{|c}{$\color{green} \uparrow $13.48} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $3.53 & $\color{green} \uparrow $17.35 & $\color{red} \downarrow $7.64 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $8.35 & $\color{green} \uparrow $16.67 & $\color{green} \uparrow $6.98 & \multicolumn{1}{|c}{$\color{green} \uparrow $8.35} & \multicolumn{1}{|c}{$\color{green} \uparrow $29.83} \\
% \cline{2-11}
%    & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $11.47 & $\color{green} \uparrow $12.35 & $\color{red} \downarrow $4.71 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $40.84 & $\color{red} \downarrow $5.88 & $\color{red} \downarrow $12.94 & \multicolumn{1}{|c}{$\color{green} \uparrow $40.84} & \multicolumn{1}{|c}{$\color{red} \downarrow $22.65} \\
%    & \multicolumn{1}{|c|}{2} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $8.24 & $\color{green} \uparrow $20.59 & $\color{green} \uparrow $5.68 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $32.78 & $\color{green} \uparrow $9.12 & $\color{red} \downarrow $5.85 & \multicolumn{1}{|c}{$\color{green} \uparrow $32.78} & \multicolumn{1}{|c}{$\color{green} \uparrow $21.30} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $12.36 & $\color{green} \uparrow $16.17 & $\color{green} \uparrow $9.43 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $36.97 & $\color{green} \uparrow $16.89 & $\color{green} \uparrow $12.65 & \multicolumn{1}{|c}{$\color{green} \uparrow $36.97} & \multicolumn{1}{|c}{$\color{green} \uparrow $42.78} \\
% \cline{2-11}
% & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $21.76 & $\color{green} \uparrow $7.94 & $\color{red} \downarrow $8.82 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $63.20 & $\color{red} \downarrow $4.41 & $\color{red} \downarrow $10.00 & \multicolumn{1}{|c}{$\color{green} \uparrow $63.20} & \multicolumn{1}{|c}{$\color{red} \downarrow $37.05} \\
%    & \multicolumn{1}{|c|}{3} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $9.98 & $\color{green} \uparrow $12.06 & $\color{red} \downarrow $15.01 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $55.78 & $\color{red} \downarrow $4.11 & $\color{red} \downarrow $14.13 & \multicolumn{1}{|c}{$\color{green} \uparrow $55.78} & \multicolumn{1}{|c}{$\color{red} \downarrow $31.17} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $11.47 & $\color{green} \uparrow $11.18 & $\color{red} \downarrow $6.76 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $55.40 & $\color{green} \uparrow $16.49 & $\color{green} \uparrow $6.81 & \multicolumn{1}{|c}{$\color{green} \uparrow $55.40} & \multicolumn{1}{|c}{$\color{green} \uparrow $16.25} \\
% \cline{2-11}
%  & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $27.94 & $\color{green} \uparrow $2.35 & $\color{red} \downarrow $11.47 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $66.15 & $\color{red} \downarrow $12.65 & $\color{red} \downarrow $12.59 & \multicolumn{1}{|c}{$\color{green} \uparrow $66.15} & \multicolumn{1}{|c}{$\color{red} \downarrow $62.30} \\
%    & \multicolumn{1}{|c|}{4} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $13.82 & $\color{green} \uparrow $13.53 & $\color{red} \downarrow $11.18 & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $58.46 & $\color{red} \downarrow $6.57 & $\color{red} \downarrow $6.47 & \multicolumn{1}{|c}{$\color{green} \uparrow $58.46} & \multicolumn{1}{|c}{$\color{red} \downarrow $24.51} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $10.12 & $\color{green} \uparrow $10.00 & $\color{red} \downarrow $4.21  & \cellcolor[HTML]{CCE4F0}$\color{green} \uparrow $61.30 & $\color{red} \downarrow $5.30 & $\color{red} \downarrow $6.74 & \multicolumn{1}{|c}{$\color{green} \uparrow $61.30} & \multicolumn{1}{|c}{$\color{red} \downarrow $16.37} \\
% \midrule
% \multirow{12}{*}{Code} & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $3.82 & $\color{green} \uparrow $7.35 & $\color{red} \downarrow $17.35 & $\color{green} \uparrow $9.12 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $10.46 & $\color{red} \downarrow $7.29 & \multicolumn{1}{|c}{$\color{green} \uparrow $10.46} & \multicolumn{1}{|c}{$\color{red} \downarrow $11.99} \\
% & \multicolumn{1}{|c|}{1} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $3.76 & $\color{green} \uparrow $5.09 & $\color{red} \downarrow $7.80 & $\color{green} \uparrow $7.68 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $5.23 & $\color{green} \uparrow $5.65 & \multicolumn{1}{|c}{$\color{green} \uparrow $5.23} & \multicolumn{1}{|c}{$\color{green} \uparrow $6.86} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $5.06 & $\color{green} \uparrow $11.82 & $\color{red} \downarrow $8.76 & $\color{green} \uparrow $8.96 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $5.98 & $\color{green} \uparrow $8.19 & \multicolumn{1}{|c}{$\color{green} \uparrow $5.98} & \multicolumn{1}{|c}{$\color{green} \uparrow $15.15} \\
% \cline{2-11}
%    & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $9.71 & $\color{red} \downarrow $6.47 & $\color{red} \downarrow $7.94 & $\color{green} \uparrow $5.29 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $47.28 & $\color{red} \downarrow $6.18 & \multicolumn{1}{|c}{$\color{green} \uparrow $47.28} & \multicolumn{1}{|c}{$\color{red} \downarrow $25.01} \\
%    & \multicolumn{1}{|c|}{2} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $7.90 & $\color{green} \uparrow $13.49 & $\color{red} \downarrow $9.05 & $\color{green} \uparrow $12.03 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $38.31 & $\color{red} \downarrow $17.76 & \multicolumn{1}{|c}{$\color{green} \uparrow $38.31} & \multicolumn{1}{|c}{$\color{red} \downarrow $9.19} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $12.22 & $\color{green} \uparrow $15.04 & $\color{green} \uparrow $6.78 & $\color{green} \uparrow $16.28 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $39.77 & $\color{green} \uparrow $6.14 & \multicolumn{1}{|c}{$\color{green} \uparrow $39.77} & \multicolumn{1}{|c}{$\color{green} \uparrow $32.02} \\
% \cline{2-11}
% & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $22.35 & $\color{red} \downarrow $8.82 & $\color{red} \downarrow $14.12 & $\color{green} \uparrow $7.94 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $61.95 & $\color{red} \downarrow $10.02 & \multicolumn{1}{|c}{$\color{green} \uparrow $61.95} & \multicolumn{1}{|c}{$\color{red} \downarrow $47.37} \\
%    & \multicolumn{1}{|c|}{3} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $9.96 & $\color{red} \downarrow $15.07 & $\color{red} \downarrow $8.46 & $\color{green} \uparrow $5.33 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $55.62 & $\color{red} \downarrow $10.04 & \multicolumn{1}{|c}{$\color{green} \uparrow $55.62} & \multicolumn{1}{|c}{$\color{red} \downarrow $38.20} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $17.39 & $\color{green} \uparrow $17.25 & $\color{red} \downarrow $9.09 & $\color{green} \uparrow $12.31 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $56.12 & $\color{green} \uparrow $6.19 & \multicolumn{1}{|c}{$\color{green} \uparrow $56.12} & \multicolumn{1}{|c}{$\color{green} \uparrow $9.27} \\
% \cline{2-11}
%  & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{100\% Specific Domain} & $\color{red} \downarrow $26.18 & $\color{red} \downarrow $7.06 & $\color{red} \downarrow $8.82 & $\color{red} \downarrow $3.24 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $64.76 & $\color{red} \downarrow $22.65 & \multicolumn{1}{|c}{$\color{green} \uparrow $64.76} & \multicolumn{1}{|c}{$\color{red} \downarrow $67.95} \\
%    & \multicolumn{1}{|c|}{4} & \multicolumn{1}{|c|}{Uniform Distribution of Non-Target Domains} & $\color{red} \downarrow $14.01 & $\color{red} \downarrow $13.86 & $\color{red} \downarrow $6.57 & $\color{green} \uparrow $6.66 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $58.06 & $\color{red} \downarrow $13.93 & \multicolumn{1}{|c}{$\color{green} \uparrow $58.06} & \multicolumn{1}{|c}{$\color{red} \downarrow $41.71} \\
%   & \multicolumn{1}{|c|}{ } & \multicolumn{1}{|c|}{\ours} & $\color{red} \downarrow $5.66 & $\color{green} \uparrow $4.42 & $\color{red} \downarrow $10.10  & $\color{green} \uparrow $9.95 & \cellcolor[HTML]{AECFD4}$\color{green} \uparrow $59.71 & $\color{red} \downarrow $13.57 & \multicolumn{1}{|c}{$\color{green} \uparrow $59.71} & \multicolumn{1}{|c}{$\color{red} \downarrow $14.96} \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{tab:flexible_domain_expansion}
% Results of \ours on flexible domain expansion, 
% % we compare the performances of several methods across different models. 
% we computed the average percentage change across various models for each method.
% ``Sum. (\%)'' denotes the total percentage of performance variations across all target and non-target domain tasks. The symbols ${\color{green} \uparrow}$ and ${\color{red} \downarrow}$ indicate an increase or decrease in the percentage of scores (\%) compared to the \textit{initial state} before supervised fine-tuning. The current target domain is highlighted using the corresponding domain color as depicted in \Cref{fig:pipeline}.}
% \end{table*}

==> chapters/implementation.tex <==
% 总述
\ours offers a comprehensive solution for data composition aimed at enhancing performance across multiple domains.  
In this section, we will briefly discuss the implementation of key components and the setting of hyperparameters.

% 在对 target model 进行 domain knowledge detection 的时候，我们使用 qwen2.5-72B chat 作为 priority model，对于每个待 fine-tune 的 target model, 我们使用 <BOS> token 作为 prompt 使其生成 40K 个 data sample，然后使用 priority model 对生成的 data sample 判断其属于各个 vertical domain (包括 law, medicine, finance, science, code, other) 的概率分数。为了保证统计结果的稳定性，我们将上述过程重复了 5 次取各轮 knowledge distribution 的均值。实际上，在sample number 为 40K 的情况下，每轮中 target model 生成的 sequence 所属各个 domain 的比例较为稳定，总体浮动不超过 1.874\% 。最终我们检测出各个 open-source model 的领域知识分布如图 3 的 stacked bar chart 所示。
\textbf{Domain Knowledge Detection.} 
During the knowledge distribution detection phase for our target models, we employed Qwen2.5-72B-Instruct\footnote{https://huggingface.co/Qwen/Qwen2.5-72B-Instruct} as the proprietary model $M_P$. For each target model $M_\theta$ slated for fine-tuning, we prompted the generation of $40K$ data samples using the Beginning of Sequence ($<BOS>$) token, with the sample number set at $N_S = 40,000$. These samples were subsequently assessed by the proprietary model $M_P$ to ascertain their probabilistic affinity for several domains, including \textit{law}, \textit{medicine}, \textit{finance}, \textit{science}, \textit{code}, and \textit{others}. To ensure the reliability of our statistical outcomes, the entire process was iterated 5 times, with the maximum number of iterations set at $T = 5$. The average knowledge distribution was then computed across these iterations. Empirically, with a dataset of $40K$ samples, the distribution of sequences generated by $M_\theta$ across domains demonstrated a high degree of consistency, with an overall variance not exceeding 1.874\%. The final domain knowledge distribution for each open-source model is depicted in the stacked bar chart presented in \Cref{fig:knowledge_detection_stacked_bar_chart}. 
The pre-existing domain knowledge distribution varies among different models. Therefore, it is essential to develop a data composition strategy that is tailored to the specific model being trained.

% 在对 LLM 进行多领域任务微调时，我们将 algorithm 2 和 algorithm 3 中的 number of training steps 设置为 4 epoch，magnitude of adjustment 我们尝试了 [0.1, 0.2, 0.5, 0.8, 1.0]，我们发现各个 domain 的权重顺序是具有一致性的，且均优于我们想要对比的 baseline (详细描述见 section experiment)。综合实验结果，我们将 magnitude of adjustment 选定为 0.5。此外，在 domain expansion 的场景下，综合各个模型的领域权重分布，我们将每次 target domain 的增长幅度设置为 5\%。variation threshold $\varepsilon$ 则体现了对于特定 domain 技能的提升程度与其余 non-target domain 能力损失之间的权衡，这里我们将其权重设置为 1.
\textbf{Hyper-Parameters Setting.} 
During the multi-domain task fine-tuning of LLMs, we configured the number of training steps $T$ in \Cref{alg:multi_ability} and \Cref{alg:domain_expansion} to 4 epochs. We experimented with various magnitude of adjustment, specifically $\left[0.1, 0.3, 0.5, 0.8, 1.0 \right]$, and observed consistent weight ordering across domains, which far outperformed our baselines (detailed in \Cref{subsec:baselines}). Based on these experimental outcomes, we set the magnitude of adjustment $\sigma $ to $0.5$. 
Additionally, in the context of domain expansion, we set the increment for the target domain $\delta$ to $10\%$ per training step, considering the overall domain weight distribution across models. The variation threshold, denoted as $\varepsilon$, reflects the trade-off between enhancing specific domain skills and mitigating the loss of capabilities in non-target domains, where we assigned a weight of $1$.


% Additionally, in the context of domain expansion, we set the increment for the target domain to 5\% based on the overall distribution of domain weights across the models. The variation threshold  balances the improvement in specific domain skills against the performance degradation in non-target domains. 


==> chapters/intro.tex <==
% introduction

% LLM 总体概述 → SFT 的意义 && 痛点
Large Language Models (LLMs) have become a cornerstone in Artificial Intelligence (AI)~\cite{achiam2023gpt,dwivedi2021artificial,lewkowycz2022solving}, particularly for Natural Language Processing tasks~\cite{brown2020language,devlin2018bert,radford2019language}, 
% 不同 vertical domain
reshaping AI research and applications in domains such as law~\cite{cui2023chatlaw}, medicine~\cite{singhal2023large,thirunavukarasu2023large}, finance~\cite{li2023large,wu2023bloomberggpt}, science~\cite{beltagy2019scibert,taylor2022galactica} and code~\cite{liu2024your,roziere2023code}. 
% 为了获得各 domain 的能力，需要进行 SFT
In order to further incentivize capabilities in these areas, LLMs typically undergo supervised fine-tuning (SFT) stages on specific datasets.


% 目前已有的 SFT 策略侧重于对单一 task 的微调 → 掌握多种能力的 LLM 研究十分重要
As demonstrated by the robust performances of proprietary LLMs such as GPT-4~\cite{achiam2023gpt} and Gemini~\cite{team2023gemini}, LLMs have the potential to master multiple tasks across all specific domains within a single model. 
However, most existing research on SFT tends to merely concentrate on a single ability of LLMs~\cite{dong2023abilities,xu2024large}. 
% Therefore, it is crucial to investigate the general performance of SFT with composite datasets of vertical domains and to address the challenges posed by data combinations during the SFT phase. 
% Addressing these challenges is essential for further enhancing the comprehensive capabilities of LLMs. 
We try to enhance the overall multitasking performance of LLMs across various domains by optimizing data mixing ratios during the SFT phase: 

% \begin{quote}
% \em
% How to design a data composition strategy during LLMs' SFT stages that could achieve overall multitasking capabilities? 
% \end{quote}

\begin{quote}
\em
How to design a data composition strategy that could achieve overall multitasking capabilities? 
\end{quote}

% versatile
Through extensive experimental analysis, we identified that the challenges associated with data composition strategies stem from the following three key aspects:
% Simultaneously, considering the current strategies for data composition during SFT stages, it has led to the following three challenges:


% 3 challenges
\textbf{\textit{C1: Catastrophic Forgetting.}} 
% Considering the fundamental differences between tasks across various domains, single-domain SFT of pretrained language models can easily lead to catastrophic forgetting of knowledge from other domains, which hinders the versatile fine-tuning performance of a model across multiple abilities~\cite{de2021continual,yuan2022hype}. 
% Similarly, in multi-domain SFT, the sequential training strategy of specific domain datasets in multiple stages can also result in LLMs' catastrophic forgetting of prior knowledge~\cite{dong2023abilities}. 
Given the fundamental differences between tasks across various domains, for multi-domain SFT, the sequential training strategy of specific datasets in multiple phases can easily lead to significant performance drop of prior knowledge, which is well-known as Catastrophic Forgetting~\cite{kaushik2021understanding,mccloskey1989catastrophic}.
This problem hinders the versatile fine-tuning performance of a model across multiple abilities~\cite{de2021continual,dong2023abilities,yuan2022hype}. 
% 可以补充一个实验
Therefore, mixing data from different domains is crucial for mitigating catastrophic forgetting during the SFT stage, enhancing the overall performance and adaptability. 


\textbf{\textit{C2: Low Efficiency.}} 
Existing research on data composition during the SFT phase for LLMs is still in its initial stages, with most strategies based on heuristic rules~\cite{albalak2024survey,dubey2024llama,wang2023data}. 
Such approaches struggle to optimally balance different domains, failing to maximize the overall training effectiveness for multiple abilities. 
There lacks a well-defined methodology that efficiently enhances the versatile capabilities of LLMs across multiple domains during the SFT stage.


% 现有的方法在针对某一领域的专项能力进行 SFT 时，都是事先根据经验固定好不同 specific datasets 的数据占比的。这样的策略无法根据 LLM 的实时反馈表现来动态调整当前阶段的 domain 数据配比，从而尽可能减小当前 LLM 对于其余领域任务的能力损失。
\textbf{\textit{C3: Low Flexibility in Domain Expansion.}} 
Existing SFT approaches for specific domain abilities typically pre-determine the proportions of different datasets according to prior experience~\cite{azerbayev2023llemma,roziere2023code}. Such strategies lack the flexibility to dynamically adjust the data mixing ratios of domains during the current phase based on real-time feedback from the LLMs, which hampers the ability to minimize the loss of performances in other domains as the LLMs undergo specialized training.


To address these challenges, we introduce \textbf{\textit{VersaTune}}, a novel data composition framework designed for enhancing models' overall performances across different vertical domains during fine-tuning. 
We first detect the proportion distribution of domain knowledge within the target model (\Cref{subsec:knowledge_distribution_detection}), followed by data composition based on the existing distribution for multi-ability enhancement (\Cref{subsec:effective_multi_ability_fostering}) as well as flexible domain expansion (\Cref{subsec:flexible_domain_expansion}). 
\ours exhibits the following properties:

\begin{itemize}
    \item \textbf{Efficient.} \ours employs distribution consistency training of the domain knowledge proportion during models' fine-tuning stage, providing an efficient strategy for enhancing versatile capabilities (\textbf{C2}).
    \item \textbf{Flexible.} \ours can be flexibly adapted to scenarios that expand performance on specific domain tasks while minimizing the degradation of the model's capabilities in non-target domains (\textbf{C1, C3}).
    \item \textbf{Robust.} The data composition strategy demonstrates significant improvements after fine-tuning in open-source models with parameter sizes ranging from 7B-14B, adding to the effectiveness of \ours.
    % \item \textbf{Generalized.} 可以泛化到不同的 knowledge 分类体系中 (future work?)
\end{itemize}

We evaluate our \ours on 12 downstream tasks across vertical domains, including law, medicine, finance, science, and code, as well as comprehensive datasets, each of which features two benchmarks. The results show that \ours can achieve an improvement of $35.21\%$ in versatile fine-tuning across multiple domains. Furthermore, when focusing on specific-domain fine-tuning, \ours maintains the training effectiveness in the target domain while reducing the performance degradation in other non-target domains by $38.77\%$.

==> chapters/observation_and_insight.tex <==
% 灾难性遗忘 + 学习阈值

In this section, we make a deep analysis of the model's performances on multiple domains during traditional fine-tuning, and provide some insights when designing our solution \ours.

\subsection{Observations on LLM Fine-Tuning}



\begin{figure*}[ht]
    % \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=1\textwidth]{figures/catastrophic_forgetting_v2.pdf}}
    \caption{Illustration of \textbf{\textit{Catastrophic Forgetting}}.}
    \label{fig:pipeline}
    \end{center}
    % \vskip -0.2in
\end{figure*}

% \subsection{Obstacles}

\textbf{\textit{O1. Catastrophic Forgetting.}}

\textbf{\textit{02. Low Effectiveness of Data Composition.}}



\subsection{Problem Formulation}





\begin{figure*}[ht]
    % \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=1\textwidth]{figures/pipeline.pdf}}
    \caption{Illustration of \textbf{\textit{VersaTune}}. 
    We commence by probing the knowledge distribution within the base model $M_\theta$, utilizing a proprietary model $M_P$ to estimate the probability of sequences generated by $M_\theta$ belonging to various domains, including law, medical, finance, science, code, and others. This allows us to deduce the current knowledge domain distribution in the pretrained model $M_\theta$ through an aggregation of multiple data sample classifications. Throughout the process of efficient fine-tuning, we dynamically adjust the data domain ratios in response to $M_\theta$'s real-time performance feedback, which encompasses learnable potential and forgetting degree serving as evaluative metrics, for both overall capability enhancement and flexible domain expansion, across different training steps. }
    % During this phase, we employ the learnable potential as an evaluative metric for the model's overall capability enhancement in multi-domain tasks. Additionally, we utilize the forgetting degree and learnable potential as flexible expansion indicators for fine-tuning the model's capabilities specifically within certain domains.
    \label{fig:pipeline}
    \end{center}
    % \vskip -0.2in
\end{figure*}

==> chapters/preliminary.tex <==
% \subsection{Background for LLMs}
% \label{subsec:LLM_background}

% \subsection{Transformer Models}

% Transformers were initially introduced to address sequence modeling and transduction challenges, including language modeling and machine translation~\cite{vaswani2017attention}. The core of each Transformer layer consists of self-attention mechanisms and point-wise feed-forward networks. 
% \textit{Self-attention network} enables the model to assess the importance of various words in a sequence regardless of their positions~\cite{zhang2019self}. It calculates a score for each word, indicating the degree of attention to be directed towards other sequence parts during encoding. This process involves query, key, and value weight sets that are optimized through training. 
% \textit{Feed-forward network (FFN)} applies the same linear transformation with a ReLU activation to each position individually. The FFN's role is to independently transform each position's representation, introducing non-linearity into the model and allowing it to learn complex functions~\cite{miao2022galvatron}. This component complements the self-attention mechanism by processing each input position in isolation, thus enhancing the model's adaptability to diverse data types and tasks. 
% These operations, predominantly dense algebraic computations such as matrix multiplications, lead to significant computational expenses and memory demands.


\subsection{LLMs Training}

\textit{Large Language Models (LLMs)} are Transformer-based models containing an extensive parameter count in the billions or greater, which are trained on a vast scale of datasets~\cite{zhao2023survey}. 
The training process of LLMs generally involves the pretraining and fine-tuning stages. We have outlined several concepts about LLMs training.

\subsubsection{Pretraining}

% \textbf{\textit{Pretraining.}} \quad
Large Language Models (LLMs) establish basic knowledge abilities, including language understanding and text generation, during the pretraining stage~\cite{brown2020language}. 
In this stage, LLMs engage in unsupervised training through the processing of extensive raw text corpora, thereby enhancing their capabilities in language modeling. For a given sequence $\mathrm {\textbf{x}} = \{x_1, x_2, ..., x_n\}$, the typical task for LLMs involves the prediction of the subsequent token $x_i$ given the preceding tokens $\mathrm {\textbf{x}}_{< i}$ as contextual input. The goal is to maximize the likelihood function presented in \Cref{eq:pretraining}:
\begin{gather}
\mathcal{L} _{LLM}^{PT}(\mathrm {\textbf{x}}) = \sum_{i=1}^{n}\log{P(x_i|\mathrm {\textbf{x}}_{< i})}
\label{eq:pretraining}
\end{gather}

\begin{figure}[t]
    % \vskip 0.2in
    \begin{center}
    % \centerline{\includegraphics[width=\linewidth]{figures/preliminary_versatune.pdf}}
    \includesvg[width=1\linewidth]{figures/preliminary_versatune.svg}
    \caption{An illustration of the LLMs training workflow. During the pretraining phase, raw documents are concatenated into a sequence for LLMs using special tokens such as <BOS> (Beginning of Sequence) and <EOS> (End of Sequence), thereby endowing the LLM with fundamental language generation capabilities. In the fine-tuning phase, the model's abilities in various domains are further enhanced.}
    \label{fig:preliminary}
    \end{center}
    \vskip -0.2in
\end{figure}

% caption
% 这里我们展示了在使用单一 domain data 进行 fune-tuning 的情况下，模型在其余 non-target domain 任务上的能力变化情况。Left (a) 的堆叠组柱状图展示了各个 non-target domain 能力随着 training step 变化的细节，每个组中从左到右的 5 个堆叠柱状图分别代表使用的 training dataset 来源于 law, medicine, finance, science 和 code 的情况。Right (b) 给出了使用单一domain dataset 进行训练时其余所有 non-target domains 的能力变化折线图，折线的颜色代表当前所使用的 training dataset 所来源的 domain。
% \begin{figure*}[ht]
%     % \vskip 0.2in
%     \begin{center}
%     % \centerline{\includegraphics[width=1\textwidth]{figures/catastrophic_forgetting_v2.pdf}}
%     \includesvg[width=1\linewidth]{figures/catastrophic_forgetting_v2.svg}
%     \caption{Illustration of variations in models' performance on non-target domain tasks when trained using a single-domain dataset. 
%     The grouped, stacked bar chart on the left (a) illustrates the detailed changes in performance across various non-target domains as training progresses. 
%     Each group of stacked bars, from left to right, represents the use of training datasets from \textit{law}, \textit{medicine}, \textit{finance}, \textit{science}, and \textit{code}, respectively. 
%     The line chart on the right (b) shows the overall performance changes in all non-target domains. The color of each line indicates the domain from which the training dataset was sourced.
%    }
%     \label{fig:catastrophic_forgetting}
%     \end{center}
%     \vskip -0.2in
% \end{figure*}




% \textbf{\textit{Beginning of Sequence}}  \textbf{(\textit{<BOS>})} \quad 
\hypertarget{BOS}{\textbf{\textit{Beginning of Sequence}}  \textbf{(\textit{<BOS>})}} \quad
During the above process, the Beginning of Sequence (<BOS>) token plays an important role, which serves as a signal to the model that the input sequence is starting~\cite{brown2020language,li2023trocr,wu2025grit}. It can be thought of as a special marker that indicates the start of a new sequence, allowing the model to reset its context and begin processing a new piece of text. 
In the context of pretraining, the <BOS> token is used to initialize the input to the model, and it can be concatenated with the actual text data to form the input sequence. This token helps the model to differentiate between the start of a new input and the continuation of an existing one. It is particularly crucial in tasks where \textit{the model needs to generate text} or understand the beginning of a new sentence or document, which helps the model to learn the boundaries of text sequences and to better model the statistical properties of the language data it is trained on.
The use of <BOS> tokens, along with other special tokens like \textit{<EOS> (End of Sequence)}, helps the model to learn the boundaries of text sequences and to better model the statistical properties of the language data it is trained on.


\subsubsection{Supervised Fine-Tuning}

% \textbf{\textit{Supervised Fine-Tuning.}} \quad
% SFT 总体介绍
The Supervised Fine-Tuning (SFT) stage involves further training on the pretrained model to refine it task-solving capabilities and ensure greater alignment with human instructions across multiple domains~\cite{zhao2023survey,nie2023angel}. 
% \textbf{\textit{Catastrophic Forgetting.}}
% single domain SFT
During the SFT phase, it is a typical practice to employ datasets specific to a particular domain for the fine-tuning of LLMs, which may lead to a decline in performance on non-target domains, a phenomenon commonly referred to as \textbf{\textit{catastrophic forgetting}}.
% our experiment
We conducted experiments on open-sourced models including LLaMA~\cite{dubey2024llama,touvron2023llama,touvron2023llama2} and Qwen~\cite{bai2023qwen,yang2024qwen2} series to assess how the model's proficiency in other domains changes when fine-tuned with data from a single domain, as illustrated in \Cref{tab:catastrophic_forgetting} and \Cref{fig:catastrophic_forgetting}. 
We have regulated the number of training instances per epoch to a fixed count of 10,000. 
More details about training and evaluation settings can be found in \Cref{subsec:experimental_setup}. 
Our findings indicate that when a model is trained exclusively with data from a single domain, its performance on tasks from other domains tends to degrade progressively over the course of training.


% other multi-ability SFT research && drawback
While recent research has delved into exploring fine-tuning methods for multi-task enhancement~\cite{dong2023abilities,sanh2021multitask}, they are still in their early stages. 
% , with much to be understood about the complexities involved in optimizing LLMs for diverse tasks. 
However, as shown by proprietary models such as GPT-4~\cite{achiam2023gpt} and Gemini~\cite{team2023gemini}, which exhibit outstanding multi-task performance, improving a model's versatile capabilities across various domains during the SFT phase is crucial. Therefore, our work systematically investigates methods to \textit{enhance multi-domain performance} during the SFT stage to bridge this gap.





% multi-task 介绍一下？(不同 vertical domain knowledge)

% \subsection{Transformer Architecture}

% Transformers are designed to address sequence modeling and transduction tasks, such as language modeling and machine translation~\cite{vaswani2017attention}. 
% At the heart of their architecture lie self-attention networks and point-wise feed-forward networks, which are integral to each layer. 
% These models perform dense algebraic operations, including matrix multiplications, which incurs significant computational and memory demands.

% \textbf{\textit{Self-Attention Network.}} \quad
% Self-attention stands for a critical component of the Transformer architecture, allowing the model to weigh the importance of different words in a sequence, irrespective of their positions~\cite{zhang2019self,Galvatron2023, vaswani2017attention}.  For each word in a sequence, self-attention computes a score that represents how much focus to place on other parts of the input sequence when encoding that specific word. This mechanism involves three sets of weights: query, key, and value, which are learned during training. Mathematically, self-attention can be described as a mapping of a query and a set of key-value pairs to an output, where the output is a weighted sum of the values. Each weight assigned to a value is computed by a compatibility function of the query with the corresponding key. This allows the Transformer to capture complex dependencies and relationships within the data, making it highly effective for tasks that require an understanding of the entire sequence, such as text translation or summarization.


% \textbf{\textit{Feed-Forward Network.}} \quad
% Each transformer layer includes a position-wise feed-forward network (FFN), which is applied to each position separately and identically. This consists of two linear transformations with a ReLU activation in between. The purpose of the FFN is to transform the representation independently at each position with the same, learned linear transformation. This means that while the self-attention layers share information across positions in the input, the feed-forward network processes each position independently. This component is crucial as it introduces non-linearity into the model, enabling it to learn more complex functions. Moreover, it ensures that the Transformer can adapt to different data types and tasks, providing additional flexibility and power to the model~\cite{vaswani2017attention}.

% % Following the self-attention mechanism, the feed-forward layer acts to refine and transform the contextualized representations. 
% % Every Transformer layer contains a fully connected feed-forward network, which is applied to each position independently with two linear transformations separated by a non-linear activation function, typically ReLU (Rectified Linear Unit) or GELU (Gaussian Error Linear Unit)~\cite{vaswani2017attention}.

% \subsection{LLMs Training}

% Large Language Models (LLMs) denote Transformer-based architectures equipped with hundreds of billions (or more) of parameters~\cite{zhao2023survey}, initially introduced to address sequence modeling and transduction challenges. 
% Below, we have outlined several key concepts about LLMs training.

% % \paragraph{Pre-training}
% \textbf{\textit{Pretraining.}} \quad
% The pretraining phase of LLMs is a crucial period for developing their general knowledge capabilities. During this phase, LLMs undergo unsupervised training with large-scale raw text to cultivate their language modeling skills. 
% Given a sequence $\mathrm {\textbf{x}} = \{x_1, x_2, ..., x_n\}$, the primary training task for LLMs at this stage is to predict subsequent tokens $x_i$ based on preceding tokens $\mathrm {\textbf{x}}_{< i}$ as context, outlined in \cref{fig:preliminary}.
% % next token prediction
% The objective function aims to maximize the likelihood of \Cref{eq:pretraining}.
% \begin{gather}
% \mathcal{L} _{LLM}^{PT}(\mathrm {\textbf{x}}) = \sum_{i=1}^{n}\log{P(x_i|\mathrm {\textbf{x}}_{< i})}
% \label{eq:pretraining}
% \end{gather}
% % \paragraph{Continue Pre-training}
% \textbf{\textit{Continual Pretraining.}} \quad 
% Continual pretraining is a phase that extends the initial pretraining, using the same objective as shown in \Cref{eq:pretraining}. 
% The key distinction is that  continual pretraining builds on an already trained model rather than starting from scratch.
% At this stage, the LLM has basic language modeling capabilities; the aim now is to enhance its specialized functions, such as \textit{long context modeling}, leveraging the foundational skills acquired during the initial pretraining phase. This phase is increasingly seen as a practical approach to improving model performance without the exorbitant computational costs associated with starting anew, as argued in recent studies~\cite{ibrahim2024simple,gupta2023continual,parmar2024reuse}.

% % \paragraph{Context Window}
% \textbf{\textit{Context Window.}} \quad
% The context window is the span of text that a model actively considers when predicting the next word or deciphering the text’s structure. This window defines the range of contextual neighbors used in calculating vector representations~\cite{lison2017redefining}. 
% During both the pretraining and continual pretraining phases, raw texts from various documents are \textit{concatenated} to form a continuous sequence that matches the length of the context window. Any text exceeding this length is \textit{truncated}. The size of the context window is pivotal, as it directly impacts the model’s capacity for language comprehension and generation.


% % cross-document attention
% % \textbf{\textit{Cross-Document Attention.}} \quad 
% % Self-attention modules constitute the foundational elements of each Transformer layer, predominantly involving dense algebraic operations such as matrix multiplications, which lead to substantial computational demands and memory usage~\cite{Galvatron2023}. 
% % In the pretraining and continual pretraining process of most LLMs, the scope of self-attention mechanism spans each context window, thereby inducing cross-document attention during the concatenation of different documents~\cite{ding2024fewer,pouransari2024dataset}. 

% \begin{figure}[t]
%     \centering
%     \includesvg[width=0.95\linewidth]{figures/preliminary.svg}
%     \caption{An illustration of the data processing workflow, training task, context window and self-attention mechanism. 
%     % During LLMs' pretraining and continual pretraining stages, 
%     }
%     \label{fig:preliminary}
% \vspace{-4mm}
% \end{figure}


% \begin{figure*}[t]
%     \centering
%     % \includesvg[width=\textwidth]{figures/domain_normalized_stacked_bar_chart_new.svg}
%     \includesvg[width=\textwidth]{figures/domain_balance.svg}
%     % \caption{Distribution of token counts for individual documents across different domains. Domains are arranged in descending order from top to bottom based on the proportion of documents with token numbers exceeding 64K. Documents within the domains of books and academic papers predominantly feature medium to long lengths (L $\ge$ 16K), in contrast to other fields, especially web-sourced data, where document lengths are almost exclusively below 4K.}
%     \caption{An illustration on the shortage of long documents across multiple domains.
%     \textbf{Left}: The length distribution of individual documents across various domains, arranged in descending order by the proportion of documents exceeding 64K tokens. Documents, such as \textit{books} and \textit{academic papers} predominantly conist of medium to long lengths (L $\ge$ 16K), whereas other domains, particularly \textit{web-sourced data}, contain documents almost exclusively shorter than 4K tokens.
%     \textbf{Right}: The proportion of each domain in the overall training dataset. }
%     \label{fig:domain_stacked_barchart}
% \end{figure*}

% \begin{table*}[t]
%     % \resizebox{\textwidth}{!}{
%         \centering
%         \caption{
%         % Token statistics among domains. We conducted an analysis of the maximum, minimum, and average token counts from different domains following tokenization. Data sourced from the web tends to have a shorter average length, necessitating the concatenation of multiple documents to achieve extended sequences suitable for long-context training.
%         Token statistics across domains. We analyzed the maximum, minimum, and average token counts for different domains. 
%         % Web-sourced data generally exhibits shorter average lengths, often requiring the concatenation of multiple documents to create extended sequences suitable for long-context training.
%         }
%         \label{tab:domain_token_stats}
%         \begin{tabular}{ccccccccc}
%             \toprule
%             Domain & \multicolumn{1}{|c}{Book (Chinese)} & Book (English) & Paper (English) & Code & Paper (Chinese) & Web (English) & Web (Chinese) & Others \\
%             \midrule
%             Max Len & \multicolumn{1}{|c}{24,203,838} & 8,241,838 & 10,721,906 & 1,000,000 & 1,471,297 & 1,267,049 & 80,688 & 21,839 \\
%             Min Len & \multicolumn{1}{|c}{667} & 322 & 127 & 173 & 696 & 289 & 132 & 23 \\
%             Avg Len & \multicolumn{1}{|c}{176,156} & 216,969 & 20,555 & 2,578 & 6,216 & 886 & 358 & 224 \\
%             \bottomrule
%         \end{tabular}
%     % }
% \end{table*}


% \subsection{\fontsize{10.5}{11.5}\selectfont Multi-Objective Combinatorial Optimization}
% \label{subsec:MOCO_pre}


% The multi-objective combinatorial optimization (MOCO) problem involves optimizing several objectives simultaneously, which typically conflict with each other~\cite{ulungu1994multi} and can be formulated as:
% \begin{align}  
% \max_{x \in \chi } \mathbf{f} \left( x\right) & := \left( f_1\left( x\right ), f_2\left( x\right ),...,f_m\left( x\right )\right ) \nonumber \\  
% \text{s.t. } & g_k \left(x\right) \le b_k + \epsilon_k, k=1,...,n  
% \label{eq:emoco}
% \end{align}
% where $x$ denotes a solution in the decision space $\chi \subset \mathbb{R}^n$, $\mathbf{f}: \chi \to \mathbb{R}^m$ represents an $m$-dimensional vector-valued objective function, and $g_k \left(x\right) \le b_k + \epsilon_k \, \text{where} \,  k=1,...,n $ stands for a series of soft constraints. Importantly, the evaluation process is computationally expensive for each individual objective $f_i\left(x\right), i = 1, ..., m$. 
% The complexity of MOCO challenges lies in the fact that improving the outcome of one objective often leads to the deterioration of another, making it necessary to find a balance or trade-off between them.



==> chapters/related_work_old.tex <==
% SFT → 突出 multi-ability 的数据混合 (移到 preliminary 中)
% \textbf{Supervised Fine-Tuning of LLMs.} 
% % SFT 总体介绍
% The Supervised Fine-Tuning (SFT) stage of a Large Language Model (LLM) involves further training to refine the model's task-solving capabilities and ensure greater alignment with human instructions~\cite{zhao2023survey}. 
% % multi-ability
% While recent research has delved into exploring fine-tuning methods for multi-task enhancement~\cite{dong2023abilities,sanh2021multitask}, they are still in their early stages. 
% However, as shown by proprietary models such as GPT-4~\cite{achiam2023gpt} and Gemini~\cite{team2023gemini}, which exhibit outstanding multi-task performance, improving a model's versatile capabilities across various domains during the SFT phase is crucial. Therefore, our work systematically investigates methods to enhance multi-domain performance during the SFT stage.


\textbf{Data Reweighting for LLM Training.}
Data reweighting maintains full access to the entire dataset while adjusts the relative importance of each instance for various target tasks, which is essential for both pretraining and fine-tuning stages of LLMs~\cite{wang2023data}. 
% pretraining stage
During the pretraining stage, DoReMi~\cite{xie2024doremi} and DoGE~\cite{fan2023doge} employ lightweight proxy models to estimate weights for different data sources, which are subsequently applied to the formal training of LLMs. 
Furthermore, Sheared LLaMA~\cite{xia2023sheared} implements an online variant of DoReMi, where the loss reference provided by the proxy model is replaced with the state of the pre-trained model from the previous training step. 
Additionally, ODM~\cite{albalak2023efficient} leverages the differences in loss or perplexity across domains within a multi-armed bandit framework to dynamically adjust the data distribution along training steps. 
% fine-tuning stage
As for the SFT phase, Dong et al.~\cite{dong2023abilities} focus on enhancing the model's math reasoning, coding, and general human-aligning abilities through a dual-stage mixed fine-tuning strategy. However, the mixing ratios for different domains rely heavily on enumeration and empirical methods, and the covered domains are not holistic. 
% ~\cite{dong2023abilities}
This paper provides a comprehensive overview of the model's capabilities across various domains during the SFT stage and proposes appropriate multi-ability fine-tuning methods.


\textbf{Knowledge Detection in LLMs.} 
Investigating the knowledge contained in current LLMs is essential for guiding their subsequent training~\cite{chang2024survey}. The knowledge encompasses multiple dimensions, such as different domain sources and task attributes. 
Existing work in LLM knowledge detection primarily focuses on prompting and calibration. Directly prompting the model to generate sequences and extracting confidence scores from the model~\cite{gekhman2024does,kadavath2022language,kuhn2023semantic,manakul2023selfcheckgpt} is a common strategy. However, such approaches are highly dependent on prompt design and task selection, which can introduce bias into the assessment. 
Other studies have attempted to infer the training data mixtures used in previous training stages of LLMs~\cite{antoniades2024generalization,hayase2024data,hu2022membership,ye2022enhanced}. The essence of these studies is to evaluate the current knowledge state of the models and provide targeted strategies for data organization and management in subsequent training phases.


==> chapters/table.tex <==
\begin{table}[h]
    \centering
    \caption{Results of law related tasks on multi-ability fostering.}
    \label{tab:multi_ability_law}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cccc}
            \toprule
            Model & Method & \multicolumn{1}{|c}{LawBench} & LegalBench \\
            \midrule
           \multirow{3}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
            \bottomrule
        \end{tabular}
    }
\end{table}

\begin{table}[h]
    \centering
    \caption{Results of medical tasks on multi-ability fostering.}
    \label{tab:multi_ability_results_medical}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cccc}
            \toprule
            Model & Method & \multicolumn{1}{|c}{MedBench} & MedMCQA \\
            \midrule
           \multirow{3}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 39.53 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 44.93 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 7.60 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 13.55 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 14.51 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
            \bottomrule
        \end{tabular}
    }
\end{table}


\begin{table}[h]
    \centering
    \caption{Results of science related tasks on multi-ability fostering.}
    \label{tab:multi_ability_results_science}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cccc}
            \toprule
            Model & Method & \multicolumn{1}{|c}{SciEval} & MMLU-Sci \\
            \midrule
           \multirow{3}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
            \bottomrule
        \end{tabular}
    }
\end{table}


\begin{table}[h]
    \centering
    \caption{Results of code related tasks on multi-ability fostering.}
    \label{tab:multi_ability_results_code}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cccc}
            \toprule
            Model & Method & \multicolumn{1}{|c}{HumanEval} & BigCodeBench \\
            \midrule
           \multirow{3}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
            \bottomrule
        \end{tabular}
    }
\end{table}


\begin{table}[h]
    \centering
    \caption{Results of general tasks on multi-ability fostering.}
    \label{tab:multi_ability_results_general}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cccc}
            \toprule
            Model & Method & \multicolumn{1}{|c}{AGIEval} & Hellaswag \\
            \midrule
           \multirow{3}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 71.4 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & 71.33^{\color{red} \downarrow } \\
          & \ours & \multicolumn{1}{|c}{xxx} & \textbf{71.76}^{\color{green} \uparrow } \\
          \midrule
           \multirow{3}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 73.26 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & 72.4^{\color{red} \downarrow } \\
          & \ours & \multicolumn{1}{|c}{xxx} & \textbf{73.62}^{\color{green} \uparrow } \\
          \midrule
           \multirow{3}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 69.8 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & 69.59^{\color{red} \downarrow } \\
          & \ours & \multicolumn{1}{|c}{xxx} & \textbf{71.51}^{\color{green} \uparrow } \\
          \midrule
           \multirow{3}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 73.6 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & 73.52^{\color{red} \downarrow } \\
          & \ours & \multicolumn{1}{|c}{xxx} & \textbf{73.67}^{\color{green} \uparrow } \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & 73.69 \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & 72.92^{\color{red} \downarrow } \\
          & \ours & \multicolumn{1}{|c}{xxx} & \textbf{73.9}^{\color{green} \uparrow } \\
          \midrule
           \multirow{3}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
          \midrule
           \multirow{3}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          &  Inverse Distribution & \multicolumn{1}{|c}{xxx} & xxx \\
          & \ours & \multicolumn{1}{|c}{xxx} & xxx \\
            \bottomrule
        \end{tabular}
    }
\end{table}

==> chapters/table_old.tex <==
\begin{table}[]
\centering
\caption{Results of law related tasks on multi-ability fostering.}
\label{tab:law}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
        \toprule
        Model & Method & \multicolumn{1}{|c}{LegalBench} & LawBench \\
        \midrule
       \multirow{4}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{15.71} & 30.72 \\
      &  Inverse Distribution & \multicolumn{1}{|c}{13.23$^{\color{red} \downarrow }$} & 26.94$^{\color{red} \downarrow }$ \\
      &  \ours Constant & \multicolumn{1}{|c}{\underline{21.47}$^{\color{green} \uparrow }$} & \underline{35.55}$^{\color{green} \uparrow }$ \\
      & \ours & \multicolumn{1}{|c}{\textbf{23.18}$^{\color{green} \uparrow }$} & \textbf{36.31}$^{\color{green} \uparrow }$ \\
      \midrule
       \multirow{4}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{33.52} & 31.16 \\
      &  Inverse Distribution & \multicolumn{1}{|c}{27.83$^{\color{red} \downarrow }$} & 27.48$^{\color{red} \downarrow }$ \\
      &  \ours Constant & \multicolumn{1}{|c}{\underline{47.85}$^{\color{green} \uparrow }$} & \underline{37.75}$^{\color{green} \uparrow }$ \\
      & \ours & \multicolumn{1}{|c}{\textbf{49.67}$^{\color{green} \uparrow }$} & \textbf{37.87}$^{\color{green} \uparrow }$ \\
      % \midrule
      %  \multirow{4}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{30.33} & 33.49 \\
      % &  Inverse Distribution & \multicolumn{1}{|c}{29.80$^{\color{red} \downarrow }$} & 30.13$^{\color{red} \downarrow }$ \\
      % &  \ours Constant & \multicolumn{1}{|c}{\underline{37.97}$^{\color{green} \uparrow }$} & \underline{35.52}$^{\color{green} \uparrow }$ \\
      % & \ours & \multicolumn{1}{|c}{\textbf{40.04}$^{\color{green} \uparrow }$} & \textbf{35.95}$^{\color{green} \uparrow }$ \\
      \midrule
       \multirow{4}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{39.05} & 31.99 \\
      &  Inverse Distribution & \multicolumn{1}{|c}{34.01$^{\color{red} \downarrow }$} & 27.81$^{\color{red} \downarrow }$ \\
      &  \ours Constant & \multicolumn{1}{|c}{\underline{45.86}$^{\color{green} \uparrow }$} & \underline{32.72}$^{\color{green} \uparrow }$ \\
      & \ours & \multicolumn{1}{|c}{\textbf{50.56}$^{\color{green} \uparrow }$} & \textbf{35.54}$^{\color{green} \uparrow }$ \\
      \midrule
       \multirow{4}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{40.11} & 31.48 \\
      &  Inverse Distribution & \multicolumn{1}{|c}{36.36$^{\color{red} \downarrow }$} & 26.98$^{\color{red} \downarrow }$ \\
      &  \ours Constant & \multicolumn{1}{|c}{\underline{48.78}$^{\color{green} \uparrow }$} & \underline{35.20}$^{\color{green} \uparrow }$ \\
      & \ours & \multicolumn{1}{|c}{\textbf{51.65}$^{\color{green} \uparrow }$} & \textbf{36.75}$^{\color{green} \uparrow }$ \\
      \midrule
       \multirow{4}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{47.66} & 34.85 \\
      &  Inverse Distribution & \multicolumn{1}{|c}{40.12$^{\color{red} \downarrow }$} & 30.67$^{\color{red} \downarrow }$ \\
      &  \ours Constant & \multicolumn{1}{|c}{\underline{53.79}$^{\color{green} \uparrow }$} & \underline{38.73}$^{\color{green} \uparrow }$ \\
      & \ours & \multicolumn{1}{|c}{\textbf{55.87}$^{\color{green} \uparrow }$} & \textbf{40.14}$^{\color{green} \uparrow }$ \\
      \midrule
       \multirow{4}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{50.73} & 39.49 \\
      &  Inverse Distribution & \multicolumn{1}{|c}{46.08$^{\color{red} \downarrow }$} & 35.36$^{\color{red} \downarrow }$ \\
      &  \ours Constant & \multicolumn{1}{|c}{\underline{56.94}$^{\color{green} \uparrow }$} & \underline{45.64}$^{\color{green} \uparrow }$ \\
      & \ours & \multicolumn{1}{|c}{\textbf{60.59}$^{\color{green} \uparrow }$} & \textbf{46.58}$^{\color{green} \uparrow }$ \\
        \bottomrule
\end{tabular}
}
\end{table}


\begin{table}[]
\centering
\caption{Results of medical tasks on multi-ability fostering.}
\label{tab:medicine}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
                \toprule
                Model & Method & \multicolumn{1}{|c}{MedQA} & MedMCQA \\
                \midrule
               \multirow{4}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{23.45} & 27.57 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{21.38$^{\color{red} \downarrow }$} & 26.52$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{30.17}$^{\color{green} \uparrow }$} & \underline{36.72}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{35.04}$^{\color{green} \uparrow }$} & \textbf{40.75}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{31.03} & 10.26 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{25.51$^{\color{red} \downarrow }$} & 8.77$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{37.33}$^{\color{green} \uparrow }$} & \underline{30.15}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{42.21}$^{\color{green} \uparrow }$} & \textbf{45.72}$^{\color{green} \uparrow }$ \\
              % \midrule
              %  \multirow{4}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{21.27} & 12.14 \\
              % &  Inverse Distribution & \multicolumn{1}{|c}{16.15$^{\color{red} \downarrow }$} & 9.91$^{\color{red} \downarrow }$ \\
              % &  \ours Constant & \multicolumn{1}{|c}{\underline{25.60}$^{\color{green} \uparrow }$} & \underline{30.28}$^{\color{green} \uparrow }$ \\
              % & \ours & \multicolumn{1}{|c}{\textbf{30.47}$^{\color{green} \uparrow }$} & \textbf{32.24}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{35.07} & 17.73 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{23.90$^{\color{red} \downarrow }$} & 16.31$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{40.89}$^{\color{green} \uparrow }$} & \underline{39.13}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{45.48}$^{\color{green} \uparrow }$} & \textbf{41.24}$^{\color{green} \uparrow }$ \\
              \midrule
              \multirow{4}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{25.17} & 25.84 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{24.16$^{\color{red} \downarrow }$} & 19.35$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{30.20}$^{\color{green} \uparrow }$} & \underline{49.71}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{34.28}$^{\color{green} \uparrow }$} & \textbf{52.09}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{32.98} & 36.54 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{26.27$^{\color{red} \downarrow }$} & 28.78$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{40.69}$^{\color{green} \uparrow }$} & \underline{42.74}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{45.78}$^{\color{green} \uparrow }$} & \textbf{47.67}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{47.85} & 38.71 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{45.75$^{\color{red} \downarrow }$} & 32.56$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{48.11}$^{\color{green} \uparrow }$} & \underline{41.64}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{50.24}$^{\color{green} \uparrow }$} & \textbf{45.15}$^{\color{green} \uparrow }$ \\
                \bottomrule
            \end{tabular}
}
\end{table}


\begin{table}[]
\centering
\caption{Results of finance related tasks on multi-ability fostering.}
\label{tab:finance}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
                \toprule
                Model & Method & \multicolumn{1}{|c}{FinEval} & FinanceIQ \\
                \midrule
               \multirow{4}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{33.50} & 2.71 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{32.96$^{\color{red} \downarrow }$} & 2.53$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{35.89}$^{\color{green} \uparrow }$} & \underline{6.28}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{36.27}$^{\color{green} \uparrow }$} & \textbf{29.04}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{34.83} & 4.97 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{33.71$^{\color{red} \downarrow }$} & 3.31$^{\color{red} \downarrow }$ \\
               &  \ours Constant & \multicolumn{1}{|c}{\underline{37.93}$^{\color{green} \uparrow }$} & \underline{25.27}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{38.80}$^{\color{green} \uparrow }$} & \textbf{43.58}$^{\color{green} \uparrow }$ \\
              % \midrule
              %  \multirow{4}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{53.87} & 14.17 \\
              % &  Inverse Distribution & \multicolumn{1}{|c}{53.80$^{\color{red} \downarrow }$} & 12.44$^{\color{red} \downarrow }$ \\
              % &  \ours Constant & \multicolumn{1}{|c}{\underline{55.06}$^{\color{green} \uparrow }$} & \underline{37.52}$^{\color{green} \uparrow }$ \\
              % & \ours & \multicolumn{1}{|c}{\textbf{55.52}$^{\color{green} \uparrow }$} & \textbf{56.63}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{59.49} & 14.62 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{56.53$^{\color{red} \downarrow }$} & 11.30$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{60.63}$^{\color{green} \uparrow }$} & \underline{40.82}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{60.95}$^{\color{green} \uparrow }$} & \textbf{68.39}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{59.58} & 31.66 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{57.07$^{\color{red} \downarrow }$} & 29.25$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\textbf{62.94}$^{\color{green} \uparrow }$} & \underline{48.47}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\underline{62.48}$^{\color{green} \uparrow }$} & \textbf{69.09}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{37.54} & 32.85 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{36.67$^{\color{red} \downarrow }$} & 26.76$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{39.33}$^{\color{green} \uparrow }$} & \underline{38.47}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{39.48}$^{\color{green} \uparrow }$} & \textbf{55.12}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{64.72} & 64.39 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{64.88$^{\color{green} \uparrow }$} & 60.53$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{65.03}$^{\color{green} \uparrow }$} & \underline{73.24}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{65.84}$^{\color{green} \uparrow }$} & \textbf{78.68}$^{\color{green} \uparrow }$ \\
                \bottomrule
            \end{tabular}
}
\end{table}


\begin{table}[]
\centering
\caption{Results of science related tasks on multi-ability fostering.}
\label{tab:science}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
                \toprule
                Model & Method & \multicolumn{1}{|c}{SciEval} & MMLU-Sci \\
                \midrule
               \multirow{4}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{9.30} & 42.89 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{8.98$^{\color{red} \downarrow }$} & 39.67$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{49.91}$^{\color{green} \uparrow }$} & \underline{45.87}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{56.75}$^{\color{green} \uparrow }$} & \textbf{50.06}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{6.51} & 50.17 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{6.09$^{\color{red} \downarrow }$} & 46.62$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{54.77}$^{\color{green} \uparrow }$} & \underline{56.04}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{56.67}$^{\color{green} \uparrow }$} & \textbf{60.61}$^{\color{green} \uparrow }$ \\
              % \midrule
              %  \multirow{4}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{7.63} & 50.67 \\
              % &  Inverse Distribution & \multicolumn{1}{|c}{6.54$^{\color{red} \downarrow }$} & 48.52$^{\color{red} \downarrow }$ \\
              % &  \ours Constant & \multicolumn{1}{|c}{\underline{38.39}$^{\color{green} \uparrow }$} & \underline{57.33}$^{\color{green} \uparrow }$ \\
              % & \ours & \multicolumn{1}{|c}{\textbf{47.76}$^{\color{green} \uparrow }$} & \textbf{61.11}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{25.30} & 62.73 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{18.57$^{\color{red} \downarrow }$} & 58.25$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{45.93}$^{\color{green} \uparrow }$} & \underline{67.29}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{51.58}$^{\color{green} \uparrow }$} & \textbf{70.42}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{19.88} & 65.84 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{16.68$^{\color{red} \downarrow }$} & 62.78$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{56.04}$^{\color{green} \uparrow }$} & \underline{71.96}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{68.14}$^{\color{green} \uparrow }$} & \textbf{74.16}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{45.72} & 50.77 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{38.96$^{\color{red} \downarrow }$} & 48.68$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{57.13}$^{\color{green} \uparrow }$} & \underline{55.10}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{63.87}$^{\color{green} \uparrow }$} & \textbf{62.84}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{39.74} & 73.45 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{27.68$^{\color{red} \downarrow }$} & 68.22$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{48.31}$^{\color{green} \uparrow }$} & \underline{78.46}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{62.89}$^{\color{green} \uparrow }$} & \textbf{82.86}$^{\color{green} \uparrow }$ \\
                \bottomrule
            \end{tabular}
}
\end{table}


\begin{table}[]
\centering
\caption{Results of code related tasks on multi-ability fostering.}
\label{tab:code}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
                \toprule
                Model & Method & \multicolumn{1}{|c}{HumanEval} & MBPP \\ % BigCodeBench
                \midrule
               \multirow{4}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{5.67} & 3.44 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{3.47$^{\color{red} \downarrow }$} & 2.42$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{12.47}$^{\color{green} \uparrow }$} & \underline{14.47}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{15.62}$^{\color{green} \uparrow }$} & \textbf{15.68}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{22.94} & 28.85 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{19.67$^{\color{red} \downarrow }$} & 24.34$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\textbf{29.88}$^{\color{green} \uparrow }$} & \underline{33.22}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\underline{28.91}$^{\color{green} \uparrow }$} & \textbf{35.65}$^{\color{green} \uparrow }$ \\
              % \midrule
              %  \multirow{4}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{32.86} & 25.86 \\
              % &  Inverse Distribution & \multicolumn{1}{|c}{28.55$^{\color{red} \downarrow }$} & 23.94$^{\color{red} \downarrow }$ \\
              % &  \ours Constant & \multicolumn{1}{|c}{\underline{38.41}$^{\color{green} \uparrow }$} & \underline{29.67}$^{\color{green} \uparrow }$ \\
              % & \ours & \multicolumn{1}{|c}{\textbf{40.49}$^{\color{green} \uparrow }$} & \textbf{31.80}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{53.26} & 37.82 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{50.65$^{\color{red} \downarrow }$} & 33.63$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{56.71}$^{\color{green} \uparrow }$} & \underline{45.87}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{58.15}$^{\color{green} \uparrow }$} & \textbf{47.64}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{55.64} & 46.86 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{52.97$^{\color{red} \downarrow }$} & 44.63$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{59.15}$^{\color{green} \uparrow }$} & \underline{52.10}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{60.68}$^{\color{green} \uparrow }$} & \textbf{61.25}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{36.54} & 38.55 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{28.78$^{\color{red} \downarrow }$} & 35.83$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{42.74}$^{\color{green} \uparrow }$} & \underline{42.76}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{47.67}$^{\color{green} \uparrow }$} & \textbf{44.62}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{68.75} & 72.14 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{63.36$^{\color{red} \downarrow }$} & 68.49$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{78.72}$^{\color{green} \uparrow }$} & \underline{78.33}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{82.64}$^{\color{green} \uparrow }$} & \textbf{81.48}$^{\color{green} \uparrow }$ \\
                \bottomrule
        \end{tabular}
}
\end{table}


\begin{table}[]
\centering
\caption{Results of general tasks on multi-ability fostering.}
\label{tab:general}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
                \toprule
                Model & Method & \multicolumn{1}{|c}{AGIEval} & HellaSwag \\
                \midrule
               \multirow{4}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{20.16} & 71.40 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{18.83$^{\color{red} \downarrow }$} & 71.33$^{\color{red} \downarrow }$ \\
              &  \ours Constant & \multicolumn{1}{|c}{\underline{22.31}$^{\color{green} \uparrow }$} & \textbf{71.89}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{24.67}$^{\color{green} \uparrow }$} & \underline{71.76}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{23.87} & 73.26 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{23.45$^{\color{red} \downarrow }$} & 72.40$^{\color{red} \downarrow }$ \\
               &  \ours Constant & \multicolumn{1}{|c}{\underline{25.62}$^{\color{green} \uparrow }$} & \underline{73.33}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{28.78}$^{\color{green} \uparrow }$} & \textbf{73.62}$^{\color{green} \uparrow }$ \\
              % \midrule
              %  \multirow{4}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{39.19} & 69.80 \\
              % &  Inverse Distribution & \multicolumn{1}{|c}{39.56$^{\color{green} \uparrow }$} & 69.59$^{\color{red} \downarrow }$ \\
              %  &  \ours Constant & \multicolumn{1}{|c}{\underline{42.50}$^{\color{green} \uparrow }$} & \underline{70.67}$^{\color{green} \uparrow }$ \\
              % & \ours & \multicolumn{1}{|c}{\textbf{42.96}$^{\color{green} \uparrow }$} & \textbf{71.51}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{47.31} & \underline{73.60} \\
              &  Inverse Distribution & \multicolumn{1}{|c}{45.74$^{\color{red} \downarrow }$} & 73.52$^{\color{red} \downarrow }$ \\
               &  \ours Constant & \multicolumn{1}{|c}{\textbf{48.16}$^{\color{green} \uparrow }$} & 72.98$^{\color{red} \downarrow }$ \\
              & \ours & \multicolumn{1}{|c}{\underline{48.02}$^{\color{green} \uparrow }$} & \textbf{73.67}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{45.42} & 73.69 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{45.67$^{\color{green} \uparrow }$} & 72.92$^{\color{red} \downarrow }$ \\
               &  \ours Constant & \multicolumn{1}{|c}{\underline{47.75}$^{\color{green} \uparrow }$} & \underline{73.88}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{49.73}$^{\color{green} \uparrow }$} & \textbf{73.90}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{36.89} & 73.50 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{36.67$^{\color{red} \downarrow }$} & 73.11$^{\color{red} \downarrow }$ \\
               &  \ours Constant & \multicolumn{1}{|c}{\underline{37.91}$^{\color{green} \uparrow }$} & \underline{74.27}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{39.64}$^{\color{green} \uparrow }$} & \textbf{74.63}$^{\color{green} \uparrow }$ \\
              \midrule
               \multirow{4}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{54.92} & 75.88 \\
              &  Inverse Distribution & \multicolumn{1}{|c}{54.87$^{\color{red} \downarrow }$} & 75.42$^{\color{red} \downarrow }$ \\
               &  \ours Constant & \multicolumn{1}{|c}{\underline{55.04}$^{\color{green} \uparrow }$} & \textbf{76.45}$^{\color{green} \uparrow }$ \\
              & \ours & \multicolumn{1}{|c}{\textbf{55.52}$^{\color{green} \uparrow }$} & \underline{75.98}$^{\color{green} \uparrow }$ \\
                \bottomrule
            \end{tabular}
}
\end{table}


\begin{table*}[tb]
    \centering
    \caption{Results of \ours on multi-ability fostering, we compare the performances of several methods across different models. The domain performance scores were calculated as the mean of respective domain benchmark scores. ``Avg.'' denotes the average performance across all domain-specific tasks. ${\color{green} \uparrow}$ and ${\color{red} \downarrow}$ indicate an increase or decrease in scores comparing to the \textbf{uniform distribution} strategy.
}
    \label{tab:multi_ability_avg}
    % \resizebox{\textwidth}{!}{
        \begin{tabular}{ccccccccc}
            \toprule
                Model & Method & \multicolumn{1}{|c}{Law} & Medical & Finance & Science & Code & \multicolumn{1}{c|}{General} & Avg. \\
            \midrule
             \multirow{3}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{23.22} & 25.51 & 18.11 & 26.10 & 4.56 & 45.78 & \multicolumn{1}{|c}{23.88} \\
              &  Inverse Distribution & \multicolumn{1}{|c}{20.09$^{\color{red} \downarrow}$} & 23.95$^{\color{red} \downarrow}$ & 17.75$^{\color{red} \downarrow}$ & 24.33$^{\color{red} \downarrow}$ & 2.95$^{\color{red} \downarrow}$ & 45.08$^{\color{red} \downarrow}$ & \multicolumn{1}{|c}{22.36$^{\color{red} \downarrow}$} \\
              & \ours & \multicolumn{1}{|c}{\textbf{29.75}$^{\color{green} \uparrow}$} & \textbf{37.90}$^{\color{green} \uparrow}$ & \textbf{32.66}$^{\color{green} \uparrow}$ & \textbf{53.41}$^{\color{green} \uparrow}$ & \textbf{15.65}$^{\color{green} \uparrow}$ & \textbf{48.22}$^{\color{green} \uparrow}$ & \multicolumn{1}{|c}{\textbf{36.27}$^{\color{green} \uparrow}$} \\
              \midrule
              \multirow{3}{*}{LLaMA-3-8B} & Uniform Distribution & \multicolumn{1}{|c}{32.34} & 20.65& 19.90& 28.34& 25.90& 48.57& \multicolumn{1}{|c}{29.28} \\
              &  Inverse Distribution & \multicolumn{1}{|c}{27.66$^{\color{red} \downarrow}$} & 17.14$^{\color{red} \downarrow}$ & 18.51$^{\color{red} \downarrow}$ & 26.36$^{\color{red} \downarrow}$ & 22.01$^{\color{red} \downarrow}$ & 47.93$^{\color{red} \downarrow}$ & \multicolumn{1}{|c}{26.60$^{\color{red} \downarrow}$} \\
              & \ours & \multicolumn{1}{|c}{\textbf{43.77}$^{\color{green} \uparrow}$} & \textbf{43.97}$^{\color{green} \uparrow}$ & \textbf{41.19}$^{\color{green} \uparrow}$ & \textbf{58.64}$^{\color{green} \uparrow}$ & \textbf{32.28}$^{\color{green} \uparrow}$ & \textbf{51.20}$^{\color{green} \uparrow}$ & \multicolumn{1}{|c}{\textbf{45.18}$^{\color{green} \uparrow}$} \\
              \midrule
              \multirow{3}{*}{Qwen-1.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{31.91} & 16.71& 34.02& 29.15& 29.36& 54.50& \multicolumn{1}{|c}{32.61} \\
              &  Inverse Distribution & \multicolumn{1}{|c}{29.97$^{\color{red} \downarrow}$} & 13.03$^{\color{red} \downarrow}$ & 33.12$^{\color{red} \downarrow}$ & 27.53$^{\color{red} \downarrow}$ & 26.25$^{\color{red} \downarrow}$ & 54.58$^{\color{red} \downarrow}$ & \multicolumn{1}{|c}{30.75$^{\color{red} \downarrow}$} \\
              & \ours & \multicolumn{1}{|c}{\textbf{38.00}$^{\color{green} \uparrow}$} & \textbf{31.36}$^{\color{green} \uparrow}$ & \textbf{56.08}$^{\color{green} \uparrow}$ & \textbf{54.44}$^{\color{green} \uparrow}$ & \textbf{36.15}$^{\color{green} \uparrow}$ & \textbf{57.24}$^{\color{green} \uparrow}$ & \multicolumn{1}{|c}{\textbf{45.55}$^{\color{green} \uparrow}$} \\
              \midrule
              \multirow{3}{*}{Qwen-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{35.52} & 26.40& 37.06& 44.02& 45.54& 60.46& \multicolumn{1}{|c}{41.50} \\
              &  Inverse Distribution & \multicolumn{1}{|c}{30.91$^{\color{red} \downarrow}$} & 20.11$^{\color{red} \downarrow}$ & 33.92$^{\color{red} \downarrow}$ & 38.41$^{\color{red} \downarrow}$ & 42.14$^{\color{red} \downarrow}$ & 59.63$^{\color{red} \downarrow}$ & \multicolumn{1}{|c}{37.52$^{\color{red} \downarrow}$} \\
              & \ours & \multicolumn{1}{|c}{\textbf{43.05}$^{\color{green} \uparrow}$} & \textbf{43.36}$^{\color{green} \uparrow}$ & \textbf{64.67}$^{\color{green} \uparrow}$ & \textbf{61.00}$^{\color{green} \uparrow}$ & \textbf{52.90}$^{\color{green} \uparrow}$ & \textbf{60.85}$^{\color{green} \uparrow}$ & \multicolumn{1}{|c}{\textbf{54.31}$^{\color{green} \uparrow}$} \\
              \midrule
             \multirow{3}{*}{Qwen-2.5-7B} & Uniform Distribution & \multicolumn{1}{|c}{35.80} & 25.51& 45.62& 42.86& 51.25& 59.56& \multicolumn{1}{|c}{43.43} \\
              &  Inverse Distribution & \multicolumn{1}{|c}{31.67$^{\color{red} \downarrow}$} & 21.76$^{\color{red} \downarrow}$ & 43.16$^{\color{red} \downarrow}$ & 39.73$^{\color{red} \downarrow}$ & 48.80$^{\color{red} \downarrow}$ & 59.30$^{\color{red} \downarrow}$ & \multicolumn{1}{|c}{40.74$^{\color{red} \downarrow}$} \\
              & \ours & \multicolumn{1}{|c}{\textbf{44.20}$^{\color{green} \uparrow}$} & \textbf{43.19}$^{\color{green} \uparrow}$ & \textbf{65.79}$^{\color{green} \uparrow}$ & \textbf{71.15}$^{\color{green} \uparrow}$ & \textbf{60.97}$^{\color{green} \uparrow}$ & \textbf{61.82}$^{\color{green} \uparrow}$ & \multicolumn{1}{|c}{\textbf{57.85}$^{\color{green} \uparrow}$} \\
              \midrule
              \multirow{3}{*}{LLaMA-2-13B} & Uniform Distribution & \multicolumn{1}{|c}{41.26} & 34.76& 35.20& 48.25& 37.55& 55.20& \multicolumn{1}{|c}{42.04} \\
              &  Inverse Distribution & \multicolumn{1}{|c}{35.40$^{\color{red} \downarrow}$} & 27.53$^{\color{red} \downarrow}$& 31.72$^{\color{red} \downarrow}$& 43.82$^{\color{red} \downarrow}$& 32.31$^{\color{red} \downarrow}$& 54.89$^{\color{red} \downarrow}$& \multicolumn{1}{|c}{37.61$^{\color{red} \downarrow}$} \\
              & \ours & \multicolumn{1}{|c}{\textbf{48.01}$^{\color{green} \uparrow}$} & \textbf{46.73}$^{\color{green} \uparrow}$& \textbf{47.30}$^{\color{green} \uparrow}$& \textbf{63.36}$^{\color{green} \uparrow}$& \textbf{46.15}$^{\color{green} \uparrow}$& \textbf{57.14}$^{\color{green} \uparrow}$& \multicolumn{1}{|c}{\textbf{51.45}$^{\color{green} \uparrow}$} \\
              \midrule
              \multirow{3}{*}{Qwen-2.5-14B} & Uniform Distribution & \multicolumn{1}{|c}{45.11} & 43.28& 64.56& 56.60& 70.45& 65.4& \multicolumn{1}{|c}{57.57} \\
              &  Inverse Distribution & \multicolumn{1}{|c}{40.72$^{\color{red} \downarrow}$} & 39.16$^{\color{red} \downarrow}$& 62.71$^{\color{red} \downarrow}$& 47.95$^{\color{red} \downarrow}$& 65.93$^{\color{red} \downarrow}$& 65.15$^{\color{red} \downarrow}$& \multicolumn{1}{|c}{53.60$^{\color{red} \downarrow}$} \\
              & \ours & \multicolumn{1}{|c}{\textbf{53.59}$^{\color{green} \uparrow}$} & \textbf{47.70}$^{\color{green} \uparrow}$& \textbf{72.26}$^{\color{green} \uparrow}$& \textbf{72.88}$^{\color{green} \uparrow}$& \textbf{82.06}$^{\color{green} \uparrow}$& \textbf{65.75}$^{\color{green} \uparrow}$& \multicolumn{1}{|c}{\textbf{65.71}$^{\color{green} \uparrow}$} \\
            \bottomrule
        \end{tabular}
    % }
\end{table*}


\begin{table*}[tb]
    \centering
    \caption{Results of \ours on multi-ability fostering, we compare the performances of several methods across different models. The domain performance scores were calculated as the mean of respective domain benchmark scores. ``Avg.'' denotes the average performance across all domain-specific tasks. ${\color{green} \uparrow}$ and ${\color{red} \downarrow}$ indicate an increase or decrease in scores comparing to the \textbf{uniform distribution} strategy.
}
    \label{tab:multi_ability_total}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{ccccccccccccccc}
            \toprule
                \multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{2}{|c}{Law} & \multicolumn{2}{|c}{Medical} & \multicolumn{2}{|c}{Finance} & \multicolumn{2}{|c}{Science} & \multicolumn{2}{|c}{Code} & \multicolumn{2}{|c|}{General} & \multirow{2}{*}{Avg.} \\
            \cline{3-14}
             & & \multicolumn{1}{|c}{LegalBench} & LawBench & \multicolumn{1}{|c}{MedQA} & MedMCQA & \multicolumn{1}{|c}{FinEval} & FinanceIQ & \multicolumn{1}{|c}{SciEval} & MMLU-Sci & \multicolumn{1}{|c}{HumanEval} & MBPP & \multicolumn{1}{|c}{AGIEval} & \multicolumn{1}{c|}{HellaSwag} & \\
            \midrule
             \multirow{4}{*}{LLaMA-2-7B} & Uniform Distribution & \multicolumn{1}{|c}{23.22} & 25.51 & 18.11 & 26.10 & 4.56 & 45.78 & \multicolumn{1}{|c}{23.88} \\
              &  Inverse Distribution & \multicolumn{1}{|c}{20.09$^{\color{red} \downarrow}$} & 23.95$^{\color{red} \downarrow}$ & 17.75$^{\color{red} \downarrow}$ & 24.33$^{\color{red} \downarrow}$ & 2.95$^{\color{red} \downarrow}$ & 45.08$^{\color{red} \downarrow}$ & \multicolumn{1}{|c}{22.36$^{\color{red} \downarrow}$} \\
               & \ours Constant & \multicolumn{1}{|c}{\textbf{29.75}$^{\color{green} \uparrow}$} & \textbf{37.90}$^{\color{green} \uparrow}$ & \textbf{32.66}$^{\color{green} \uparrow}$ & \textbf{53.41}$^{\color{green} \uparrow}$ & \textbf{15.65}$^{\color{green} \uparrow}$ & \textbf{48.22}$^{\color{green} \uparrow}$ & \multicolumn{1}{|c}{\textbf{36.27}$^{\color{green} \uparrow}$} \\
              & \ours & \multicolumn{1}{|c}{\textbf{29.75}$^{\color{green} \uparrow}$} & \textbf{37.90}$^{\color{green} \uparrow}$ & \textbf{32.66}$^{\color{green} \uparrow}$ & \textbf{53.41}$^{\color{green} \uparrow}$ & \textbf{15.65}$^{\color{green} \uparrow}$ & \textbf{48.22}$^{\color{green} \uparrow}$ & \multicolumn{1}{|c}{\textbf{36.27}$^{\color{green} \uparrow}$} \\
        \end{tabular}
    }
\end{table*}

==> chapters/versa_tune1_domain_detection.tex <==
% 总体描述
Here, we first present a domain mixing strategy for fine-tuning a LLM that possesses a comprehensive multitask capability (\Cref{subsec:knowledge_consistency_training}). This approach is designed to align with the inherent domain knowledge distribution within the base model waiting for subsequent training. Following this, we describe the method for detecting domain knowledge proportion of the base model, which is crucial for informing the fine-tuning process (\Cref{subsec:knowledge_distribution_detection}).


\subsubsection{Knowledge Consistency Training}
\label{subsec:knowledge_consistency_training}

% 之前工作的不足之处 (作为过渡)
% 之前对于 LLM SFT 阶段不同 domain 数据配比的工作大多数关注于培养 LLM 一个特定领域的能力，因此会仅仅使用该单一领域的数据，或者根据经验启发式地给出数据配比。we argue that 这样数据配比策略会严重造成 LLM 对某些领域能力的严重损失。在 SFT 阶段，LLM 对于不同 domain 的总体综合能力是非常重要的。那么什么样的数据配比策略可以有效提升 LLM SFT 阶段的各领域整体表现？我们给出了以下 statement:
Previous research on data mixing ratios during the SFT phase for LLMs has predominantly focused on enhancing capabilities within a specific domain, often utilizing only data from that domain or employing heuristic, experience-based data proportions. We argue that such strategies can significantly impair the LLM's abilities in other domains. In the fine-tuning stage, maintaining a robust overall capability across various domains is crucial. 

What data mixing strategy effectively boosts the versatile performance of LLMs across domains during the SFT phase? We propose the statement:

% 给出 domain knowledge distribution 的假设
\hypertarget{statement1}{\textbf{\textit{Statement 1}}}
% (Knowledge Consistency Training). 
\textit{An LLM fine-tuned with domain-specific data proportions $P_{SFT}(x)$ that align with its pretrained output distributions $P_{knowledge}(x)$ will exhibit enhanced and balanced performance across these domains, compared to a model fine-tuned with a non-matching data distribution. Formally, the relationship can be represented as:}

\begin{equation}
\label{eq:statement1}
    P_{SFT}(x) \approx P_{knowledge}(x), \forall x \in \chi
\end{equation}
\textit{where $\chi$ denotes the set of all possible data points.}

% % reason
% The statement is based on the fact that the model has developed a general understanding of language features and knowledge specific to various domains during the pretraining phase. Maintaining the same distribution of knowledge during fine-tuning allows the model to build on this pre-existing knowledge, enhancing learning efficiency and robustness.

% kimi
% \hypertarget{statement1}{\textbf{Statement 1}}
% \textit{An LLM fine-tuned with domain-specific data proportions that align with its pre-trained output distributions will exhibit enhanced and balanced performance across these domains compared to a model fine-tuned with a non-matching data distribution. This concept is formally represented as:}

% \begin{equation}
% \label{eq:statement1}
%     P_{SFT}(x) \approx P_{knowledge}(x), \forall x \in \chi
% \end{equation}
% \textit{where $P_{SFT}(x)$ denotes the fine-tuned model's output distribution for domain $x$, $P_{knowledge}(x)$ represents the pre-trained model's knowledge distribution for domain $x$, and $\chi$ is the set of all possible data points.}

The rationale behind this statement is rooted in the observation that during the pretraining phase, LLMs develop a general understanding of language features and domain-specific knowledge. By maintaining the same distribution of knowledge during fine-tuning, the model can build upon this pre-existing knowledge, thereby enhancing learning efficiency and robustness. 


% 待补充 (优点)
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Generalization and Robustness.} 
%     The model has developed an understanding of language features and knowledge specific to various domains during pretraining. Maintaining the same distribution of knowledge during fine-tuning allows the model to build on this pre-existing knowledge, enhancing learning efficiency and robustness.
%     % \item \textbf{Bias Minimization.} 
%     % Deviating heavily from a model's domain knowledge distribution in the fine-tuning phase might lead to strong performance in over-represented domains, but poor performance in under-represented ones. Matching the domain distribution helps avoid introducing such biases, ensuring more balanced model abilities.
%     \item \textbf{Optimal Knowledge Transfer.} 
%     By referring to models' domain knowledge distribution in the fine-tuning stage, the model is better positioned to transfer and apply its pre-trained knowledge to fine-tuning tasks. This is particularly important in domains requiring deep, specialized knowledge, such as medical and law.
% \end{itemize}


\subsubsection{Domain Knowledge Distribution Detection}
\label{subsubsec:knowledge_distribution_detection}

% Inspired by the knowledge identification methods~\cite{gekhman2024does,zhao2023knowing} and training data inference strategies~\cite{hayase2024data} of LLMs from previous work, 
% we propose a systematic approach for efficient domain knowledge detection. 
% The process involves the generation of textual outputs from the base model waiting to be fine-tuning, followed by their classification into predefined domains (e.g., law, medical, finance, science, code etc.) referring to a proprietary LLM. The above process is repeated multiple times to ensure statistical robustness. 
Drawing on prior research into knowledge identification methods~\cite{gekhman2024does,zhao2023knowing} and training data inference strategies for LLMs~\cite{CVPR_distribution_estimation,hayase2024data}, we propose a structured approach to efficiently detect domain knowledge based on statistics. 
The method involves the generation of textual outputs from the base model $M_{\theta}$ waiting for fine-tuning, followed by classification into predefined domains referring to a proprietary model $M_P$. The process is repeated multiple times to ensure statistical robustness.

% pipeline description
Assuming the data corpus contains $k$ distinct domains, 
as shown in \Cref{alg:domain_detection}, we first prompt the base model poised for fine-tuning $M_{\theta}$ with the 
% Beginning of Sequence (\textless BOS\textgreater) 
\hyperlink{BOS}{Beginning of Sequence (\textless BOS\textgreater)} 
tokens to generate a set of $N_S$ data entries 
% $\mathcal{S}=\{s_1, s_2, ..., s_{N_S}\}$. 
$\mathcal{S}=\{s_i\}_{i=1}^{N_S}$ (Line 3). 
Subsequently, we employ a proprietary model $M_P$ to infer probabilities that these $N_S$ entries belong to each domain (Line 5-7). We then calculate a weighted average of the probability distributions for all data across these domains, thereby deriving the domain knowledge distribution of the current base model $M_{\theta}$ (Line 9). To ensure statistical robustness, the process is iteratively conducted $T$ times, and we use the mean of these $T$ iterations as the estimated result for knowledge distribution.

% This methodology entails generating textual outputs from a base model poised for fine-tuning, which are then classified into predefined domains such as law, medical, finance, science, and code, referring to a proprietary LLM. To ensure statistical robustness, this classification process is iteratively conducted multiple times. 

% Beginning of Sequence (BOS): This token indicates the beginning of a sequence. It is often used in tasks such as language modeling or sequence generation to signal the model to start generating text.

% new version
% \begin{algorithm}[tb]
% \caption{Domain Knowledge Distribution Detection}
% \label{alg:domain_detection}
% \SetAlgoLined
% \SetKwProg{Fn}{Function}{}{end}
% \SetKwInput{KwData}{Input}
% \SetKwInput{KwParameter}{Parameter}
% \SetKwInput{KwDefine}{Define}
% \SetKwInput{KwResult}{Ouptut}
% \KwData{Base model to be fine-tuned $M_{\theta}$, Proprietary model $M_P$, Hyperparameters: sample number $N_S$, maximum iterations $T$}
% \KwParameter{Data samples generated from the base model $\mathcal{S}$}
% \KwResult{Domain distribution $\vec{P}$}
% \KwDefine{$\vec{p}$: domain probability distribution of data sample $s$}
% \For{$t = 1, 2, \ldots, T$}{
%     /* \textit{Step 1: Data Generation} */\;
    
%     Generate data samples from base model $\mathcal{S}=\{s_i\}_{i=1}^{N_S}$ where $s_i = M_{\theta}(\textless BOS \textgreater)$\;
    
%     /* \textit{Step 2: Domain Probability Inference} */\;
    
%     \For{each data sample $s_i$ in $\mathcal{S}$}{
%         Provide domain probability of $s_i$ referring to the proprietary model $M_P$: $\vec{p_i} = (p_{ij})_{j=1}^{k} \gets M_P(s_i)$\;
%     }
%     /* \textit{Step 3: Statistics Aggregation} */\;
    
%     Estimate the domain distribution $\vec{P}^{(t)} = (P_j^{(t)})_{j=1}^k$ where $P_j^{(t)} = \frac{1}{N_S}\sum_{i=1}^{N_S}p_{ij}$\;
% }
% \Return $\vec{P} = (P_j)_{j=1}^k$ where $P_j = \frac{1}{T}\sum_{t=1}^{T}P_j^{(t)}$\;
% \end{algorithm}


\subsection{Phase 2: Fine-Tuning Multi-Ability LLMs Efficiently}
\label{subsec:fine_tuning_multi_ability_llm}

% 总体概述
% 我们已经对 base model 中所包含的领域知识分布进行了探测，接下来我们将运用探测结果指导我们的多领域 SFT，从而使得微调后的模型最大化多领域任务的表现，并灵活地进行特定领域能力的扩展。
Having detected the distribution of domain knowledge within the base model, we will now utilize these findings to guide our multi-ability SFT process. The approaches are designed to enhance the overall performance of the fine-tuned model across a spectrum of multi-domain tasks (\Cref{subsec:effective_multi_ability_fostering}), as well as to facilitate the flexible expansion of capabilities in specific domains (\Cref{subsec:flexible_domain_expansion}).


\textbf{Setting.} 
% \quad 
Our goal is to construct a composite dataset covering $k$ specific domains, which can be 
denoted as 
% $\mathcal{D}_{train} = \{ (D_{train}^1, P_1), (D_{train}^2, P_2), ..., (D_{train}^k, P_k) \}$ 
$\mathcal{D}_{train} = \{ (D_{train}^j, P_j)\}_{j=1}^{k}$ 
with each tuple representing a specific domain and its corresponding proportion, 
% with the format of $(domain, proportion)$, 
such that training a model on dataset $\mathcal{D}_{train}$ could achieve overall lower loss on a uniformly distributed composite target validation dataset 
% $\mathcal{D}_{val} = \{ (D_{val}^1, 1 / k), (D_{val}^2, 1 / k), ..., (D_{val}^k, 1 / k) \}$, 
$\mathcal{D}_{val} = \{ (D_{val}^j, 1 / k)\}_{j=1}^{k}$ or meet the flexible domain expansion while preserving the performances in other domains. 
The specialized capabilities of LLMs are measured using downstream tasks related to different domains (e.g., FinBen~\cite{xie2024finben} for financial performances).


% original version
\begin{algorithm}[tb]
\caption{Knowledge Distribution Detection}
% \caption{Domain Knowledge Distribution Detection}
\label{alg:domain_detection}
% \begin{algorithmic}[1]
\begin{flushleft}
\textbf{Input}: Base model $M_{\theta}$, Proprietary model $M_P$, Hyperparameters: sample number $N_S$, maximum iterations $T$\\
\textbf{Parameter}: Data samples $\mathcal{S}$ generated from $M_{\theta}$ \\
\textbf{Output}: Domain distribution $\vec{P}$ \\
Define $\vec{p}$: domain probability distribution of data sample $s$ \\
\end{flushleft}
\begin{algorithmic}[1]
\FOR{$t = 1, 2, \ldots, T$}
    \STATE /* \textit{Step 1: Data Generation} */
    \STATE Generate data samples from the base model: $\mathcal{S}=\{s_i\}_{i=1}^{N_S}$ where $s_i = M_{\theta}(\textless BOS \textgreater)$
    \STATE /* \textit{Step 2: Domain Probability Inference} */
    \FOR{each data sample $s_i$ in $\mathcal{S}$}
        \STATE Provide domain probability of $s_i$ referring to the proprietary model $M_P$: \\ \quad \quad $\vec{p_i} = (p_{ij})_{j=1}^{k} \gets M_P(s_i)$
    \ENDFOR
    \STATE /* \textit{Step 3: Statistics Aggregation} */
    \STATE Estimate domain knowledge distribution: \\ \mbox{$\vec{P}^{(t)} = (P_j^{(t)})_{j=1}^k$ where $P_j^{(t)} = \frac{1}{N_S}\sum_{i=1}^{N_S}p_{ij}$}
    % \FOR{$j = 1, 2, \ldots, k$}
    %     \STATE $P_j^{(t)} \gets \frac{1}{N_S}\sum_{i=1}^{N_S}p_{ij}$
    % \ENDFOR
\ENDFOR
\STATE \mbox{\textbf{Return} $\vec{P} = (P_j)_{j=1}^k$ where $P_j = \frac{1}{T}\sum_{t=1}^{T}P_j^{(t)}$}
\end{algorithmic}
\end{algorithm}


\subsubsection{Preliminary: Learnable Potential and Forgetting Degree of Knowledge}
% \subsubsection{Learnable Potential and Forgetting Degree of Domain Knowledge}
% \subsubsection{Learnable Potential and Forgetting Degree of Knowledge}

Before formally introducing the effective multi-task fine-tuning and flexible domain expansion data composing strategies, we will first provide an overview of the evaluation metrics used for the following algorithms in this subsection.

\textbf{\textit{Mastery Ceiling.}} \quad 
We first fine-tuned the small \textit{reference model} $M_{ref}$ for $T_{ref}$ epochs on each domain separately, and identified the epoch with the lowest average loss during this process as the lower bound on the minimum loss attainable by the target model $M_\theta$ for the given domain. This value represents the highest level of domain knowledge mastery that the model can achieve in the context of the current specific domain under given conditions.

% 给出 loss 下降空间的 description
\textbf{\textit{Learnable Potential.}} \quad 
We can observe whether a domain could be effectively learned by the model through comparing the difference between the loss of the target model $M_\theta$ and the minimum loss that the reference model $M_{ref}$ can achieve. Based on these principles, we propose \Cref{eq:loss_potential} to score the learnable potential of domain $j$:

\begin{equation}
\label{eq:loss_potential}
    \gamma_j = \max \{\frac{\ell_{\theta}^{j} - \ell_{ref}^{j}}{\ell_{\theta}^{j}}, 0 \}
\end{equation}
where $\ell_{\theta}^{j}$ denotes the loss associated with the target model $M_\theta$ for the $j$-th domain, while $\ell_{ref}^{j}$ signifies the corresponding loss for the reference model $M_{ref}$ within the same domain. 
To mitigate the impact of inherent loss variations across different domains for the model, we have introduced a normalization term into the formula.


\textbf{\textit{Forgetting Degree.}} \quad 
When focusing on expanding a model to a specific domain, our objective is to minimize the loss of the model's knowledge regarding other domains. Here we segment the fine-tuning stage into $T$ distinct checkpoints. We quantify the degree of knowledge loss, or the forgetting of the current domain, by measuring the difference in loss between the $t$-th and $(t - 1)$-th training steps. This difference reflects the model's mastery loss for the tasks associated with the current domain. Based on this principle, we introduce \Cref{eq:forgetting_degree} to assess the model's forgetting degree for domain $j$ at the $t$-th training step.

\begin{equation}
\label{eq:forgetting_degree}
    \varphi_j^{(t)} = \max \{\frac{\ell_{\theta^{(t)}}^{j} - \ell_{\theta^{(t - 1)}}^{j}}{\ell_{\theta^{(t - 1)}}^{j}}, 0 \}
\end{equation}
where $\ell_{\theta^{(t)}}^{j}$ represents the loss at the $t$-th training step associated with the target model $M_\theta$ for the $j$-th domain, while $\ell_{\theta^{(t - 1)}}^{j}$ denotes the loss at the preceding $(t - 1)$-th iteration for the same domain. 
We also incorporated a normalization factor into the equation to counteract the effects of inherent loss disparities among domains.


% overall ability enhancement
\subsubsection{Effective Multi-Ability Fostering}
\label{subsec:effective_multi_ability_fostering}


\begin{algorithm}[tb]
\caption{VersaTune Multi-Ability Fine-Tuning (for Domain Robustness)}
\label{alg:multi_ability}
% \begin{algorithmic}[1]
\begin{flushleft}
\textbf{Input}: Base model to be fine-tuned $M_{\theta}^{(0)}$, Domain reference loss $\{\ell_{ref}^{j}\}_{j=1}^{k}$, Hyperparameters: adjustment magnitude $\sigma$, training step number $T$\\
\mbox{\textbf{Parameter}: Data proportion $\{P_{j}\}_{j=1}^{k}$ of SFT dataset} \\
\textbf{Output}: Fine-tuned multi-ability model $M_{\theta}^{(T)}$ \\
Define $\gamma$: learnable potential  of the current domain \\
\end{flushleft}
\begin{algorithmic}[1]
\STATE Initialize domain proportion $\{P_{j}^{(0)}\}_{j=1}^{k}$ according to \Cref{eq:statement1} and \Cref{alg:domain_detection}
\FOR{$t = 1, 2, \ldots, T$}
    % \FOR{$j$ from $1$ to $k$}
    \FOR{$j = 1, 2, \ldots, k$}
    % loss reduction scope
        \STATE Learnable potential for the $j$-th domain: \\ \quad \quad $\gamma_j^{(t)} = \max \{\frac{\ell_{\theta^{(t)}}^{j} - \ell_{ref}^{j}}{\ell_{\theta^{(t)}}^{j}}, 0 \}$
        \STATE Update domain weights: \\ \quad \quad $P_j^{(t)'} = P_j^{(t-1)}(1 + \sigma 
 \gamma_j^{(t)})$
    \ENDFOR
    % \STATE Compute the scope for loss reduction of each domain: $\gamma_j = \max \{\frac{\ell_{\theta^{(t - 1)}}^{j} - \ell_{ref}^{j}}{\ell_{\theta^{(t - 1)}}^{j}}, 0 \}$ where $j \in \{1, 2, ..., k\}$
    % \STATE Update domain weights $\{P_j^{(t)'}\}_{j=1}^k = \{P_j^{(t-1)}(1 + \sigma \gamma_j)\}_{j=1}^k$
    \STATE Renormalize domain weights: \\ \quad $P_j^{(t)} = \frac{P_j^{(t)'}}{\sum_{i=1}^{k}P_i^{(t)'}}, \quad \forall j \in \{1, 2, ..., k\}$
    \STATE \mbox{Update parameters of fine-tuned model $M_{\theta}^{(t)}$}
    % : \\ \centering{$M_{\theta}^{(t)} \gets M_{\theta}^{(t-1)}$}
\ENDFOR
\STATE \textbf{Return} Fine-tuned model $M_{\theta}^{(T)}$
\end{algorithmic}
\end{algorithm}

To cultivate the multi-tasking capabilities of a LLM during the fine-tuning phase, we have aligned the initial domain distribution in the SFT stage with the knowledge detection results of the base model as stated in \Cref{eq:statement1}. Furthermore, we dynamically make minor adjustments in the composition ratios of various domains based on the model's real-time feedback at different SFT stages. 
% This adaptive approach is employed to maximize the model's comprehensive training benefits across multiple domain tasks. 

% 我们首先在 SFT 初始阶段将 domain 的配比按照 algorithm 1 中探测出的 base model 本身的 domain knowledge 分布进行混合 (Line 1)；然后在每个检查点t，按照 equation 2 的方式对每个 domain 进行 learnable potential 打分，并以此分数为依据对当前 domain 的在整体数据集中的占比进行细微调整，以确保各个 domain 的能力在微调过程中是均衡发展的（Line 3-7）。
As detailed in \Cref{alg:multi_ability}, in the pursuit of balanced domain expertise enhancement, we first blended the domain proportions in accordance with the base model's intrinsic domain knowledge distribution detected by \Cref{alg:domain_detection} (Line 1). Then at each training step $t$, we assigned a learnable potential score to each domain based on the methodology outlined in \cref{eq:loss_potential}. These scores were then utilized to fine-tune the representation of each domain within the composite SFT dataset, ensuring a balanced development of competencies across all domains throughout the training process (Line 3-7). 
At the same time, the parameters of model $M_{\theta}$ are updated based on the gradients computed through backpropagation (Line 8).
This adaptive approach is imperative to harmonize the progression of capabilities in different domains and to optimize the model's performance on multiple tasks. 
% a multifaceted array of tasks.

==> chapters/versa_tune2_SFT.tex <==
\begin{algorithm}[ht]
\caption{VersaTune Multi-Ability Fine-Tuning (for Domain Expansion)}
\label{alg:domain_expansion}
% \begin{algorithmic}[1]
\begin{flushleft}
\textbf{Input}: Base model to be fine-tuned $M_{\theta}^{(0)}$, Domains that require enhanced cultivation $D_e$, \mbox{Domain reference loss $\{\ell_{ref}^{j}\}_{j=1}^{k}$, Hyperparameters:} \\ training step number $T$, adjustment magnitude $\sigma $, domain adjustment extent $\delta$, variation threshold $\varepsilon$ \\
\mbox{\textbf{Parameter}: Data proportion $\{P_{j}\}_{j=1}^{k}$ of SFT dataset} \\
\textbf{Output}: Fine-tuned multi-ability model $M_{\theta}^{(T)}$ \\
Define $\gamma$: learnable potential  of the current domain \\
Define $\varphi$: forgetting degree of the current domain \\
\end{flushleft}
\begin{algorithmic}[1]
\STATE Initialize domain proportion $\{P_{j}^{(0)}\}_{j=1}^{k}$ according to \Cref{eq:statement1} and \Cref{alg:domain_detection}
\FOR{$t = 1, 2, \ldots, T$}
    \FOR{$j = 1, 2, \ldots, k $} % \, (j \neq e)
        \STATE Learnable potential for the $j$-th domain: \\ \quad \quad  $\gamma_j^{(t)} = \max \{\frac{\ell_{\theta^{(t)}}^{j} - \ell_{ref}^{j}}{\ell_{\theta^{(t)}}^{j}}, 0 \}$
        \STATE Forgetting degree for the $j$-th domain: \\ \quad \quad $\varphi_j^{(t)} = \max \{\frac{\ell_{\theta^{(t)}}^{j} - \ell_{\theta^{(t - 1)}}^{j}}{\ell_{\theta^{(t - 1)}}^{j}}, 0 \}$
        \STATE Update domain weights: \\ \quad \quad $P_j^{(t)'} = P_j^{(t-1)}(1 + \sigma 
 \gamma_j^{(t)})$
    \ENDFOR
    \IF{$\frac{1}{k} \sum_{j=1, j \neq e}^{k} \varphi_j^{(t)} < \varepsilon \gamma_e^{(t)}$}
        \STATE Update specific domain weight: \\ \mbox{$P_j^{(t)} = \begin{cases}  
            P_j^{(t-1)} + \delta, \text{if} \quad j = e & \\  
            \frac{P_j^{(t)'}}{\sum_{i=1, j \neq e}^{k}P_i^{(t)'}} (1 - P_j^{(t-1)} - \delta), \text{else} &
        \end{cases}$}
    \ELSE
        \STATE Renormalize domain weights: \\ \,\, $P_j^{(t)} = \frac{P_j^{(t)'}}{\sum_{i=1}^{k}P_i^{(t)'}}, \quad \forall j \in \{1, 2, ..., k\}$
    \ENDIF
    \STATE \mbox{Update parameters of fine-tuned model $M_{\theta}^{(t)}$}
    % \STATE Update parameters of the fine-tuned model: \\ \centering{$M_{\theta}^{(t)} \gets M_{\theta}^{(t-1)}$}
\ENDFOR
\STATE \textbf{Return} Fine-tuned model $M_{\theta}^{(T)}$
\end{algorithmic}
\end{algorithm}


% 在对 pre-trained model 进行 SFT 时，有时候也会想要着重提升 model 在某一 specific domain 任务中的能力，因此需要我们的算法框架有着灵活的 domain 扩展泛化性能。基于 statement 1，我们给出了针对 domain expansion SFT 的数据配比陈述。
When conducting fine-tuning on a pretrained model, there are instances where we aim to particularly enhance models' performance on specific domain tasks. Consequently, our algorithmic framework ought to possess the flexibility to accommodate domain expansion and generalize effectively. Building upon \hyperlink{statement1}{Statement 1}, we present the following statement tailored for domain expansion:
% Derived from \hyperlink{statement1}{Statement 1}

% 给出 domain knowledge distribution 的假设
\paragraph{\textbf{Statement 2}} 
\label{para:statement2}
% 在针对 LLM 某一特殊能力进行微调时，在增加某个特定domain的数据量时，其他 domain 按照base model 所包含的 knowledge 分布进行相应的调整，可以达到灵活的 domain expansion 策略。
\textit{When fine-tuning a LLM for a specific capability, increasing the volume of data from a particular domain $D_e$ while adjusting other domains $(j = 1,2, ..., k, j \neq e)$ according to the knowledge distribution of the base model, facilitates a flexible strategy for domain expansion. Formally, the relationship can be represented as:}
% \textit{If a LLM is fine-tuned using a distribution of domain-specific data that matches the distribution observed in its pre-trained outputs across various domains, then the model will demonstrate improved and balanced performance across these domains compared to a model fine-tuned with a non-matching distribution of domain data.}

\begin{equation}
\label{eq:statement2}
    P_{SFT}^{'}(x) \approx \sum_{j=1}^{k} A(D_j) P_{SFT}(x | D_j), j = 1, 2, ..., k
\end{equation}
\textit{where $P_{SFT}(x | D_j)$ is the data distribution in the domain $D_j$, and $A(D_j)$ is the adjustment factor.}

Here $A(D_j)$ is determined based on the knowledge distribution of the pre-trained domain. In particular, when $D_e$ increases, the other domains $\{D_j\}_{j = 1, j \neq e}^{k}$ shrink proportionally as a whole, which can be expressed as:

\begin{equation}
\label{eq:statement2_cases}
    A(D_j) =
    \begin{cases}  
        \alpha, \text{if} \quad j = e & \\  
        \beta \frac{1}{\sum_{j=1, j \neq e}^{k} A(D_j)} , \text{others} &
    \end{cases} 
\end{equation}
% \text{if} \quad j = 1, 2, ..., k, j \neq e
where $\alpha$ is the increased adjustment factor, and $\beta$ is the original ratio of other domain knowledge relative to $D_e$.


% 我们同样首先按照从原始 pre-trained model 中探测出的知识分布进行初始数据配比（Line 1）。在每个 training step t，我们分别计算每个 domain 的 learnable potential 分数和 forgetting degree 分数（Line 4-5），并按照 algorithm 2 中的方法对当前阶段的数据配比进行初始化（Line 6）。我们需要在当前需要突出培养的 domain 的剩余学习上升空间与 model 对其他 domain 的遗忘程度之间做权衡：如果 specific domain 的上升效益优于其余 domain 的平均遗忘程度（比值大于 e），则对当前 specific domain 的数据权重提升 \theta，其余 domain 按照 equation 5的方法等比例减少(Line 8-9)；否则保持当前阶段的领域配比，仅按照同 algorithm 2 的方法进行权重微调并归一化（Line 10-11）。然后更新 target model 的参数（Line 13）
% As outlined in \Cref{alg:domain_expansion}, we initially establish the data distribution based on the knowledge detected from the original pretrained model (Line 1). At each training step $t$, we calculate the learnable potential and forgetting degree scores for each domain (Line 4-5), and assign domain weights for the current training phase following the method from \Cref{alg:multi_ability} (Line 6). A trade-off is necessary between the remaining learning margin of the domain that requires focused cultivation and the model's forgetting degree towards other non-target domains: if the improvement benefit of the specific domain exceeds the average forgetting degree of the other domains (ratio greater than $\varepsilon$), we increase the data weight of the current specific domain by $\delta$, and proportionally reduce the weights of the other non-target domains according to \Cref{eq:statement2_cases} (Line 8-9); otherwise, we maintain the current domain distribution and only perform minor adjustments and renormalization as described in \cref{alg:multi_ability} (Line 10-11). Subsequently, we update the parameters of the target model $M_{\theta}$ (Line 13).
% In this way, we can ensure that when the data volume of a specific domain is increased, the other domains can be adjusted according to the preset ratio, thus maintaining the consistency of the overall data distribution.

% To express the similarity between the SFT domain data distribution and the pre-trained domain knowledge distribution, and to consider flexible domain expansion, we introduce an adjustment function $A(D_j)$. This function allows us to adjust the proportion of each domain in the SFT domain based on the knowledge distribution of the pre-trained domain. In this way, we can ensure that when the data volume of a specific domain is increased, the other domains can be adjusted according to the preset ratio, thus maintaining the consistency of the overall data distribution.
